A Survey of Distributed Graph Algorithms on Massive Graphs

Distributed processing of large-scale graph data has many practical applications and has been widely studied. In recent years, a lot of distributed graph processing frameworks and algorithms have been proposed. While many efforts have been devoted to analyzing these, with most analyzing them based on programming models, less research focuses on understanding their challenges in distributed environments. Applying graph tasks to distributed environments is not easy, often facing numerous challenges through our analysis, including parallelism, load balancing, communication overhead, and bandwidth. In this paper, we provide an extensive overview of the current state-of-the-art in this field by outlining the challenges and solutions of distributed graph algorithms. We first conduct a systematic analysis of the inherent challenges in distributed graph processing, followed by presenting an overview of existing general solutions. Subsequently, we survey the challenges highlighted in recent distributed graph processing papers and the strategies adopted to address them. Finally, we discuss the current research trends and identify potential future opportunities.

==> section/challenge_old_version.tex <==
% \section{Challenge}

% \textcolor{red}{add more details to introduce challenges}





% ..........................................old version...........................................

\underline{\textit{Load Balance}}

Load balance is a basic problem in distributed systems. In an ideal situation, the computation quantity of all machines are all equivalent and the computation processes are finished at the same time. However, an unreasonable partitions may cause load imbalance and delay the total processes.

The load balance problem is much more common in graph algorithms due to their irregular computing processes. First, the workload on each vertex is dramatically different. Even all vertices are distributed on average, the total computation quantity on each machine is possibly unbalanced. Figure~\ref{fig:challenge_partition_a} shows an example. Both machines save four vertices but the left one has more edges and is much denser. Therefore, the left machine has more workloads. Besides, the load balance problem is more serious in synchronous model. This unbalanced situation will happen before each synchronous signal and all other machines should wait for the slowest one while synchronizing.

To avoid load unbalance, the critical improvement is to balance the workload of each vertex. Based on this idea, there are two main methods, \textit{Partitioning} and \textit{Scheduling}. partitioning-based methods often estimate workloads in advance and then partition all vertices, while scheduling-based methods will schedule workloads dynamically. 

$\bullet$ {Partitioning}

Distributed algorithms are based on distributed storage. Traditional distributed systems focus on balancing the storage by their size, not dense. So recent partitioning-based methods aim at detecting and partitioning dense regions. For example, a high degree vertex may have a huge computation cost since each edge will request a communication, so these hub vertices should be separated to different machines. Take Figure~\ref{fig:challenge_partition} as an example. The partition in Figure~\ref{fig:challenge_partition_a} is unbalanced since the left machine is too dense and has much more communications (13 compared to 7), though two machines all have four vertices. Figure~\ref{fig:challenge_partition_b} shows a better partition. Now two machines share a same number of vertices and a similar number of edges (11 and 9). We believe it is a more balanced partition.

Furthermore, these neighbors of hub vertices should also be partitioned among different machines \cite{DBLP:conf/www/Lin19, DBLP:journals/tpds/ChakaravarthyCM17}. Different algorithms may have various measurement of hub vertices, such as the vertex in-degree, the vertex out-degree, the degeneracy number and the core number \cite{DBLP:journals/tsc/XuCF16, DBLP:journals/tpds/PandeyWZTZLLHDL21}. Further, all nodes in one machine can be distributed evenly among its threads \cite{DBLP:journals/tpds/ChakaravarthyCM17, DBLP:journals/vldb/ZhangYWTCS17}. Some recent researches choose Subgraph-Centric or Edge-Centric model to balance data automatically, which involves more evaluation and partition algorithms, i.e., partition trees \cite{DBLP:conf/ppopp/MalekiNLGPP16, DBLP:conf/sigmod/Yu0KLLCY20, DBLP:conf/podc/Censor-HillelLV22, DBLP:conf/icpp/GiechaskielPY15}.

\begin{figure}[h]
\centering
    \begin{subfigure}{0.35\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_partition_a.pdf}
		\caption{the initial partition}
        \label{fig:challenge_partition_a}
	\end{subfigure}
\hspace{-1em}
    \begin{subfigure}{0.35\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{pic/challenge/challenge_partition_b.pdf}
		\caption{a better partition}
        \label{fig:challenge_partition_b}
	\end{subfigure}
\hspace{1em}
    \begin{subfigure}{0.25\linewidth}
		\centering
		\includegraphics[width=1.0\linewidth]{pic/challenge/challenge_partition_c.pdf}
        \vspace{1.5em}
	\end{subfigure}
 \caption{An example of the partitioning method. Yellow points are graph nodes linked by green and red edges, which are local and global communications, respectively. Figure \ref{fig:challenge_partition_a} is a partition case, where $u_1, u_2, u_3, u_4$ are assigned to one machine and $v_1, v_2, v_3, v_4$ to another. The left partition has 13 communications and the right partition has only 7, leading to unbalanced workload. A better partition is shown in Figure \label{fig:challenge_partition_b} where two machines have similar number of communications (11 and 9).}
\label{fig:challenge_partition}
\end{figure}

$\bullet$ Scheduling

Although the computation cost of each vertices can be predicted and analyzed, the distributed environment is unstable and the real processing time is quite uncertain. Instead of partitioning before the process, dynamically scheduling during the computing process is more effective. As shown in Figure \ref{fig:challenge_schedule}, some models often create a main thread to manage other threads, or a whole transaction module to schedule the computation processing \cite{DBLP:journals/tpds/BusatoB15, DBLP:journals/tos/ShuCWZLL20, DBLP:journals/tpds/KhandaSBND22, DBLP:journals/tc/MinutoliCSDLFTF22}.
Unfortunately, not all systems can support these scheduling modules, so another method is to redistribute after each iteration as a manual scheduling \cite{DBLP:journals/tpds/JainFPGA17}, which is more applicable for some disconnected graphs and easy to implement.

\begin{figure}[h]
\centering
\includegraphics[width=0.55\linewidth]{pic/challenge/challenge_schedule.pdf}
\caption{An example of the scheduling method. There is a global schedule model to balance each machine, in which a inner thread manager could schedule each thread assigned to all vertices.}
\label{fig:challenge_schedule}
\end{figure}

% The first method is to replace global communications with local communications, since the cost difference between the global and the local communication is significant.
% In BFS problem, the time complexity of a naive distributed BFS algorithm is already $O(n+m)$, with no further optimization. On the contrary, a higher degree node in one machine is likely to communicate with more nodes and more other machines, leading to more global communications. Cao, Wang, et al. saved delegates of high degree nodes in other machines to reduce some global communications \cite{DBLP:conf/ppopp/CaoWWLMYC22}.
% In SSSP problem, Maleki, Nguyen, et al. divided the whole graph into multiple subgraphs, each of which is assigned to a processor. The shortest path distance in a subgraph is computed by each processor locally and independently, decreasing global communications \cite{DBLP:conf/ppopp/MalekiNLGPP16}.


\subsubsection{Communication Overhead}
\label{sec:challenge_communication}

In the filed of processing within a distributed environment, vertices exchange communicate each other by message passing. In single-thread algorithms, message passing can be easily implemented by accessing shared memory. However, distributed algorithms split vertices and edges in different machines, which need inter-thread communication, LAN communication, or even network communication. All these communications are extremely expensive and should be take into consideration. Moreover, decentralized distributed framework may involves more communications on synchronization or other operations. These issues not only increase computational latency but can also lead to network bandwidth bottlenecks, severely affecting the overall efficiency. Owing to the potential cost of communication, many distributed algorithms are dedicated to effectively reduce communication overhead. 

$\bullet$ Communication Pruning

Communication pruning aims to reduce unnecessary communications.
The selective message-passing strategy stands as a prevalent method, which is designed by such a truth that not all vertices require the complete information from their neighbors. For instance, in some graph traversal algorithms, vertices might only need to know the state or specific attributes of their neighbors. Besides, during algorithm execution, some inactive vertices may cause some unnecessary message passing. Rather than indiscriminately broadcasting messages to every neighbors, it judiciously determines message transmission based on specific conditions or guidelines \cite{DBLP:journals/tpds/MontresorPM13, DBLP:journals/jpdc/ChanSS21, DBLP:journals/tkde/ShahrivariJ21}.
Besides, global communication typically results in expensive cost, as message needs to be transmitted across different machines. Some algorithms employ partitioning strategies to ensure that vertices only need to communicate within the partitioned scope, thereby reducing global communication \cite{DBLP:conf/bigdataconf/ChenCC14,DBLP:conf/ppopp/CaoWWLMYC22}.
Furthermore, several studies \cite{DBLP:journals/pvldb/LiaoLJHXC22,DBLP:conf/ipps/GhoshHTKLCKG18} compute an upper bound, informed by each vertex's local data, to curtail the volume of message exchanges. Such a strategy also proves potent for early termination in iterative processes.

\begin{figure}[h]
\centering
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_communication_a.pdf}
		\caption{the initial communication}
	\end{subfigure}
\hspace{-0.5em}
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.82\linewidth]{pic/challenge/challenge_communication_b.pdf}
		\caption{tail node pruning}
        \label{fig:challenge_communication_b}
	\end{subfigure}
\hspace{0.5em}
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=1.0\linewidth]{pic/challenge/challenge_communication_c.pdf}
        \caption{duplicate node method}
        \label{fig:challenge_communication_c}
	\end{subfigure}
 \caption{Several examples of communication pruning. First, a better partition can reduce global communications (from 5 to 4). Then, Figure \ref{fig:challenge_communication_b} prune a tail node, which is often useless in subsequent iterations, and further reduce another global communication. Figure \ref{fig:challenge_communication_c} add two duplicate node $u_1'$ and $u_4'$. There neighbors can communicate the duplicate copy locally, instead of a global communication.}
\end{figure}

$\bullet$ Subgraph-Centric

The Subgraph-Centric method is also a strategy to reduce communication overhead in distributed systems \cite{DBLP:conf/usenix/LakhotiaKP18, DBLP:journals/tpds/MontresorPM13, DBLP:conf/sigmod/ShaoCC14}. In distributed environments, communication between machines is often substantially slower than within a single machine.
In the Subgraph-Centric framework, a computing node stores a set of vertices, with communication between subgraphs happening after computation within a subgraph converges. This method, compared to the more common Vertex-Centric framework, not only reduces communication, especially cross-machine communication, but also balances the workload among vertices.
Besides, some vertices in a subgraph can sometimes achieve local convergence within a single round, eliminating the need for constant communication with vertices in other subgraphs.

\begin{figure}[h]
\centering
    \begin{subfigure}{0.4\linewidth}
		\centering
		\includegraphics[width=0.65\linewidth]{pic/challenge/challenge_subgraph_a.pdf}
		\caption{the vertex-centric model}
	\end{subfigure}
    \begin{subfigure}{0.4\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{pic/challenge/challenge_subgraph_b.pdf}
		\caption{the subgraph-centric model}
	\end{subfigure}
 \caption{An example of the subgraph-centric model. There are three subgraphs, $\{u_1, u_2, v_2\}$, $\{v_1, v_4\}$ and $\{u_3, v_3, u_4\}$. These subgraphs are further assigned to two machines. Note the communication in the subgraph now will become random-access, so there are one global communication and three global communications in total.}
\end{figure}

$\bullet$ Aggregation

The fundamental concept of aggregation strategy is to centralize related data or information in a single location (vertex or edge), thereby alleviating the communication burden within a distributed system.
Some algorithms \cite{DBLP:conf/podc/Censor-HillelLV22, DBLP:conf/sc/BulucM11, DBLP:conf/ipps/Lamm022} consolidate the key information of vertices or edges within a specific region onto a single vertex or edge. During distributed processing, by exclusively accessing and processing the primary vertices or edges, most of the data is skipped, which not only minimizes communication overhead but also augments algorithmic efficiency. 
Furthermore, some studies \cite{DBLP:conf/podc/CaoFR21, DBLP:journals/vldb/ZhangYWTCS17} have reduced computational and communication overhead by seeking approximate solutions through the construction of skeleton graphs (a subgraph of the original graph that retains certain key features or structures of the original graph but has fewer vertices and edges). This can also be seen as a aggregation strategy.

\begin{figure}[h]
\centering
\includegraphics[width=0.55\linewidth]{pic/challenge/challenge_aggregation.pdf}
\caption{An example of the aggregator. The aggregator can aggregate multiple updates as a single update message and reduce communication cost. A common aggregator is the minimum and the maximum aggregator, which filter out the lowest and the highest updating value before the communication, respectively.}
\end{figure}

$\bullet$ Navigation

The navigation strategy is guided by the structure and characteristics of the graph for computation. Instead of blindly sending messages, it determines the message transmission path based on the graph's topology and the attributes of the vertices. Such a targeted communication approach reduces unnecessary message passing \cite{DBLP:conf/sc/WangCMYC22}. This optimization technique is common in traversal algorithms.
Some algorithms navigate and pinpoint the shortest paths by establishing shortcuts between center vertices, which serve as crucial navigational beacons within the network \cite{DBLP:conf/podc/CaoFR21}.
Furthermore, some algorithms harness paths within the skeleton graph, using them as guiding trajectories to steer towards vital regions in the primary graph \cite{DBLP:journals/vldb/ZhangYWTCS17}.

\begin{figure}[h]
\centering
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_navigation_a.pdf}
		\caption{the plain graph}
	\end{subfigure}
\hspace{-0.5em}
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_navigation_b.pdf}
		\caption{the graph with guideline}
	\end{subfigure}
\hspace{0.5em}
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_navigation_c.pdf}
        \caption{the graph with shortcut}
	\end{subfigure}
 \caption{An example of the navigation method. Suppose $u_1$ and $u_4$ often send messages to $v_3$ and $v_1$, respectively. The guideline method will navigate the communicating direction, while the shortcut method will add two shortcuts.}
\end{figure}

$\bullet$ Parallelism

Parallelism is also a major challenge in distributed graph computation and processing. 
Many traditional algorithms, optimized for sequential execution in single-machine environments, have inherent serialized steps that is difficult to be applied directly in the distributed environment. 
Additionally, some iterative algorithms have steps dependent on previous results, which leads to problems of data synchronization and data consistency when deployed in a distributed system, adding extra computational and communication overheads.

$\bullet$ Asynchronous

The synchronous framework is the most commonly used in distributed graph algorithms. It is more easier to implement, and it can prevent data inconsistency issues. In contrast, although the asynchronous framework might require more complex control and scheduling mechanisms to manage asynchronous updates and communication, it can further enhance the algorithm's parallelism.
Therefore, many algorithms \cite{DBLP:conf/icassp/HeW21,DBLP:journals/dc/MashreghiK21,DBLP:conf/sc/SteilRIPSP21,DBLP:journals/jpdc/RemisGAN18} have adopted the asynchronous framework to design distributed graph algorithms to enhance the algorithm's parallelism and efficiency.
The "parallel pipeline" method is a technique in which multiple independent pipelines run in parallel, with each pipeline handling the tasks assigned to it. Some algorithms, particularly those utilizing random walks, employ this method. By doing so, they reduce the necessary computational iterations, thereby speeding up the entire calculation process \cite{DBLP:conf/www/Lin19}.

\begin{figure}[h]
\centering
    \begin{subfigure}{1.0\linewidth}
		\centering
		\includegraphics[width=0.7\linewidth]{pic/challenge/challenge_asynchronous_a.pdf}
		\caption{the synchronous flow}
        \label{fig:challenge_asynchronous_a}
	\end{subfigure}
    \begin{subfigure}{1.0\linewidth}
		\centering
		\includegraphics[width=0.7\linewidth]{pic/challenge/challenge_asynchronous_b.pdf}
		\caption{the asynchronous flow}
        \label{fig:challenge_asynchronous_b}
	\end{subfigure}

\caption{An example of synchronous and asynchronous flow including three machines $A, B, C$. The dash line means a synchronous signal. Suppose the machine $C$ will always send a message to $A$ and $B$ after each iteration. Using synchronous model shown in Figure \ref{fig:challenge_asynchronous_a}, iterations $2A$ and $2B$ should after $1C$, iterations $3A$ and $3B$ should after $2C$. If asynchronous model is applied like Figure \ref{fig:challenge_asynchronous_b}, the machine $C$ could execute two iterations continuously, while machines $A$ and $B$ can processing two batches of updating messages together in one iteration, which can significantly reduce processing time.}
\end{figure}

\subsubsection{Bandwidth}

Due to the limitations of machine hardware and network communication, bandwidth (the communication cost between a pair of vertices/subgraphs per round) cannot be infinitely large. However, in distributed graph algorithms, vertices (or subgraphs) need to frequently exchange information, especially when the scale of the graph is very large, which leads to a bottleneck of bandwidth.

$\bullet$ Pruning

The pruning strategy aims to reduce unnecessary messages in order to reduce the size of data during each round of message passing between machines. This approach can also optimize communication overhead. 
Some algorithms \cite{DBLP:conf/icalp/BonneC19} choose to send only the primary messages for reducing the amount of information. Additionally, some studies \cite{DBLP:conf/podc/Censor-HillelGL20} reduce the amount of information generation by pruning the size of the origin graph.

$\bullet$ Segmented Processing

Due to bandwidth limitations, some algorithms \cite{DBLP:conf/icml/Luo20} adopt the segmentation strategy when transferring large-scale messages, sending only a portion of the messages at a time. Although this may increase the number of communications, in some iterative algorithms, it might help in early termination of iterations, as partial data is sufficient to complete the computations and determine whether to terminate the iteration sometimes.

% \subsubsection{Approximation} 



% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\subsubsection{Trade-Off in Distributed Algorithms}

The distributed environment and algorithm process is diverse and unpredictable. Some optimizations are not suitable in all cases. Instead, users should carefully decide whether enable these optimizations, or use a hybrid model to dynamically switch optimization scheme. So these trade-off problems bring some challenges to find a best balance. 


\subsubsection{Global or Local Computation}
In distributed computing, global computation is an intuitive way to extensively exchange message or synchronizing among vertices. But global computation is an extremely expensive operation involving broadcasting and global communications. 
Many algorithms \cite{DBLP:conf/cluster/ZengY18,DBLP:conf/ipps/GhoshHTKLCKG18,DBLP:journals/pvldb/LiaoLJHXC22,DBLP:journals/tpds/MontresorPM13,DBLP:journals/tpds/WengZLPL22,DBLP:conf/bigdataconf/ChenCC14,DBLP:journals/tkde/ShahrivariJ21} are redesigned for the distributed environments by replacing global computations with more local computations, significantly boosting the parallel processing of algorithms, making them more attuned to distributed environments.

However, the cost of global and local computation is not certain in different environments and algorithms. Though local computation is inexpensive, it requires more communications and and synchronizing supersteps to ensure the consistency of the data. Users should make a trade-off whether enable such optimization.

\subsubsection{Sparse or Dense Representation}
Sparse and dense representation are two popular message-passing methods. Shown in Figure~\ref{fig:challenge_representation}, the sparse representation will passing updating message one-by-one, while the dense representation will save them in a updating vector first and then passing the whole vector. Note not all algorithms have this merge feature. A popular application is the distance vector in some traversal algorithms.

The sparse representation may has load balance problem since updating messages on different edges are highly different. A busy edge with many updates will block the whole iteration. The dense representation is developed for this scenario. These updating messages will be mapped to a updating vector. Therefore, all edges will send a same-length vector, balancing the total workload. Compared with the sparse representation, the dense representation reduces load unbalance, though the total cost has increased. It is a trade-off between the \textit{largest} cost and the \textit{total} cost. Recent work often applies a hybrid representation that using sparse representation first and enable dense representation after the update number exceeds a threshold \cite{DBLP:conf/sc/WangCMYC22}.

\begin{figure}[h]
\centering
    \begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{pic/challenge/challenge_representation_a.pdf}
		\caption{the sparse representation}
	\end{subfigure}
    \begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[width=0.8\linewidth]{pic/challenge/challenge_representation_b.pdf}
		\caption{the dense representation}
	\end{subfigure}
 \caption{An example of the sparse and dense representation. Each solid triangle is an updating message. With sparse representation, each vertex will send updating message one-by-one and same as receiving. The inclining message distributed might lead to load unbalance. If these independent messages can be aggregate as a vector (i.e., distance vector), all communications will share a same workload although add extra communication cost (vacancy in the vector marked by hollow triangle).}
 \label{fig:challenge_representation}
\end{figure}

\subsubsection{Push or Pull Model}
The push and pull are two fundamental communication paradigms. In the push model, each active vertex will \textit{push} messages to target vertices, while in the pull model, vertices will \textit{pull} possible updates from all active vertices.

The push model is efficient since it only push real messages. On the contrary in the pull model, a vertex does not know which active vertex has an update. Instead, it should pull possible updates from all active vertices. But push model centralizes all communications on active vertices, leading to unbalanced workload. Shown in Figure~\ref{fig:challenge_push}, the left machine with two active vertices holds all communications. Instead, the pull model in Figure~\ref{fig:challenge_pull} scatters these communications over all vertices.
\textcolor{red}{pull model for early stage and push model for further stage}

Since it is hard to decide which model is better, some studies \cite{DBLP:journals/tpds/ChakaravarthyCM17, DBLP:conf/sc/SteilRIPSP21} combine the strengths of both model. They use a hybrid model to automatically determine whether to use push or pull model. For instance, the push model might be a better choice for low degree; on the contrary, if the degree of the vertex is high, the pull model might perform better. Additionally, some heuristic methods \cite{DBLP:journals/tpds/ChakaravarthyCM17} can also select a better paradigm by estimating the communication volume. For the push model, the communication volume is given by the total number of edges of the vertex; for the pull model, the communication volume is given by the number of active vertices.

\begin{figure}[h]
\centering
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_push_pull_a.pdf}
		\caption{the original graph}
	\end{subfigure}
\hspace{-0.5em}
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_push_pull_b.pdf}
		\caption{the push model}
        \label{fig:challenge_push}
	\end{subfigure}
\hspace{0.5em}
    \begin{subfigure}{0.3\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pic/challenge/challenge_push_pull_c.pdf}
        \caption{the pull model}
        \label{fig:challenge_pull}
	\end{subfigure}
 \caption{An example of push-pull model. Suppose only $u_1$ and $u_4$ are active nodes and will send messages. In the push model, $u_1$ will \textit{push} updating messages to $\{v_1, v_2, u_2, u_3, u_4\}$ and $u_4$ will \textit{push} updating messages to $\{u_1, u_2, u_3, v_3\}$. In the pull model, each node will \textit{pull} updating messages from all active neighbors. As a comparison, the push model is more efficient and easy to implement, while the pull model needs to maintain active nodes. On the contrary, the pull model is more balanced, especially when many active nodes concentrate on a few machines.}
 \vspace{-2em}
\end{figure}










\begin{table}[]
\caption{Challenges and Optimization Strategies}
\small
\begin{tabular}{|l|l|l|}
\hline
\textbf{Challenge}                                & \textbf{Strategy}                                                                                                  & \textbf{Related Work}               \\ \hline
\multirow{15}{*}{Load Balance}           & \multirow{9}{*}{Partition}                                                                                & Giechaskiel   et al., 2015 \cite{DBLP:conf/icpp/GiechaskielPY15} \\
                                         &                                                                                                           & Xu et al., 2016 \cite{DBLP:journals/tsc/XuCF16}            \\
                                         &                                                                                                           & Maleki et al., 2016 \cite{DBLP:conf/ppopp/MalekiNLGPP16}       \\
                                         &                                                                                                           & Chakaravarthy et al., 2017 \cite{DBLP:journals/tpds/ChakaravarthyCM17} \\
                                         &                                                                                                           & Zhang et al., 2017 \cite{DBLP:journals/vldb/ZhangYWTCS17}         \\
                                         &                                                                                                           & Lin et al., 2019 \cite{DBLP:conf/www/Lin19}         \\
                                         &                                                                                                           & Yu et al., 2020 \cite{DBLP:conf/sigmod/Yu0KLLCY20}           \\
                                         &                                                                                                           & Pandey et al., 2021 \cite{DBLP:journals/tpds/PandeyWZTZLLHDL21}       \\
                                         &                                                                                                           & Censor-Hillel et al., 2022 \cite{DBLP:conf/podc/Censor-HillelLV22} \\ \cline{2-3} 
                                         & \multirow{5}{*}{Scheduling}                                                                               & Busato et al., 2015 \cite{DBLP:journals/tpds/BusatoB15}       \\
                                         &                                                                                                           & Jain et al., 2017 \cite{DBLP:journals/tpds/JainFPGA17}         \\
                                         &                                                                                                           & Shu et al., 2020 \cite{DBLP:journals/tos/ShuCWZLL20}          \\
                                         &                                                                                                           & Khanda et al., 2022 \cite{DBLP:journals/tpds/KhandaSBND22}       \\
                                         &                                                                                                           & Minutoli et al., 2022 \cite{DBLP:journals/tc/MinutoliCSDLFTF22}     \\ \cline{2-3} 
                                         & Dense Representation                                                                                      & Wang et al., 2022 \cite{DBLP:conf/sc/WangCMYC22}         \\ \hline
\multirow{20}{*}{Communication Overhead} & \multirow{7}{*}{Communication Pruning}                                                                    & Montresor et al., 2013 \cite{DBLP:journals/tpds/MontresorPM13}    \\
                                         &                                                                                                           & Chen et al., 2014 \cite{DBLP:conf/bigdataconf/ChenCC14}         \\
                                         &                                                                                                           & Ghosh et al., 2018 \cite{DBLP:conf/ipps/GhoshHTKLCKG18}         \\
                                         &                                                                                                           & Shahrivari et al., 2021 \cite{DBLP:journals/tkde/ShahrivariJ21}   \\
                                         &                                                                                                           & Chan et al., 2021  \cite{DBLP:journals/jpdc/ChanSS21}        \\
                                         &                                                                                                           & Cao et al., 2022 \cite{DBLP:conf/ppopp/CaoWWLMYC22}          \\
                                         &                                                                                                           & Liao et al., 2022 \cite{DBLP:journals/pvldb/LiaoLJHXC22}         \\ \cline{2-3} 
                                         & \multirow{3}{*}{Subgraph-Centric}                                                                         & Montresor et al., 2013 \cite{DBLP:journals/tpds/MontresorPM13}    \\
                                         &                                                                                                           & Shao et al., 2014 \cite{DBLP:conf/sigmod/ShaoCC14}         \\
                                         &                                                                                                           & Lakhotia et al., 2018 \cite{DBLP:conf/usenix/LakhotiaKP18}     \\ \cline{2-3} 
                                         & \multirow{2}{*}{Push-Pull Optimization}                                                                   & Chakaravarthy et al., 2017 \cite{DBLP:journals/tpds/ChakaravarthyCM17}\\
                                         &                                                                                                           & Steil et al., 2021 \cite{DBLP:conf/sc/SteilRIPSP21}        \\ \cline{2-3} 
                                         & \multirow{5}{*}{Aggregation}                                                                              & Buluç et al., 2011 \cite{DBLP:conf/sc/BulucM11}        \\
                                         &                                                                                                           & Zhang et al., 2017 \cite{DBLP:journals/vldb/ZhangYWTCS17}        \\
                                         &                                                                                                           & Cao et al., 2021 \cite{DBLP:conf/podc/CaoFR21}          \\
                                         &                                                                                                           & Censor-Hillel et al., 2022 \cite{DBLP:conf/podc/Censor-HillelLV22} \\
                                         &                                                                                                           & Lamm et al., 2022 \cite{DBLP:conf/ipps/Lamm022}         \\ \cline{2-3} 
                                         & \multirow{3}{*}{Navigation}                                                                               & Zhang et al., 2017 \cite{DBLP:journals/vldb/ZhangYWTCS17}         \\
                                         &                                                                                                           & Cao et al., 2021 \cite{DBLP:conf/podc/CaoFR21}          \\
                                         &                                                                                                           & Wang et al., 2022 \cite{DBLP:conf/sc/WangCMYC22}         \\ \hline
\multirow{12}{*}{Parallelism}            & \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Trade-off between Global and\\ Local Computation\end{tabular}} & Montresor et al., 2013 \cite{DBLP:journals/tpds/MontresorPM13}     \\
                                         &                                                                                                           & Chen et al., 2014 \cite{DBLP:conf/bigdataconf/ChenCC14}         \\
                                         &                                                                                                           & Ghosh et al., 2018 \cite{DBLP:conf/ipps/GhoshHTKLCKG18}        \\
                                         &                                                                                                           & Zeng et al., 2018 \cite{DBLP:conf/cluster/ZengY18}         \\
                                         &                                                                                                           & Shahrivari et al., 2021 \cite{DBLP:journals/tkde/ShahrivariJ21}   \\
                                         &                                                                                                           & Liao et al., 2022 \cite{DBLP:journals/pvldb/LiaoLJHXC22}         \\
                                         &                                                                                                           & Weng et al., 2022 \cite{DBLP:journals/tpds/WengZLPL22}         \\ \cline{2-3} 
                                         & \multirow{5}{*}{Asynchronous}                                                                             & Remis et al., 2018 \cite{DBLP:journals/jpdc/RemisGAN18}        \\
                                         &                                                                                                           & Lin et al., 2019 \cite{DBLP:conf/www/Lin19}          \\
                                         &                                                                                                           & He et al., 2021 \cite{DBLP:conf/icassp/HeW21}           \\
                                         &                                                                                                           & Mashreghi et al., 2021 \cite{DBLP:journals/dc/MashreghiK21}    \\
                                         &                                                                                                           & Steil et al., 2021 \cite{DBLP:conf/sc/SteilRIPSP21}        \\ \hline
\multirow{3}{*}{Bandwidth}               & \multirow{2}{*}{Pruning}                                                                                  & Bonne et al., 2019 \cite{DBLP:conf/icalp/BonneC19}         \\
                                         &                                                                                                           & Censor-Hillel et al., 2020 \cite{DBLP:conf/podc/Censor-HillelGL20} \\ \cline{2-3} 
                                         & Segmented Processing                                                                                      & Luo et al., 2020 \cite{DBLP:conf/icml/Luo20}          \\ \hline
\end{tabular}
\end{table}

==> section/sec2_Distributed_Graph_Processing.tex <==
% In the real world, a large amount of data needs to be analyzed and processed every day, such as social network data, road network data, text data, and so on. However, due to the limitations of performance and memory on a single machine, query efficiency is often not high. Therefore, dividing and deploying them to multiple machines is a very effective approach.

In the real world, there is a amount of data that requires daily analysis and processing, including social network data, road network data, and text data, among others. However, the limited performance and memory capacity of single machines often lead to inefficiencies in query processing. Therefore, dividing and deploying data across multiple machines presents a prevalent and effective solution. In this section, we first introduce the concept of a distributed system, then discuss various distributed graph processing for handling graph data and summarize their programming models through systematic classification.

% \subsection{Distributed Architecture}
\subsection{Distributed Computing System}
The distributed computing system comprises several computational units which interact with each other by explicit or implicit message passing to achieve collaborative computing \cite{DBLP:journals/csur/HeidariSCB18}.
% The distributed computing system comprises several computational units which are connected through the network to work together and finally achieve the common goal. 
In such system, data is partitioned into distinct computational units and each unit execute corresponding tasks in parallel \cite{DBLP:journals/tpds/Jiang16}. 
Typically, the underlying hardware of a distributed system consists of a series of comparable workstations or personal computers that are closely linked by means of a high-speed network \cite{DBLP:journals/computing/SteenT16}. 
And a computational unit consists of four core components: local storage for offloading data to local disks, distributed storage to share and manage data, communication layers to facilitate inter-unit messaging, and the computing module that perform the processing tasks \cite{DBLP:journals/ftdb/YanBTD17}.
Due to the characteristics of high availability, scalability, fault tolerance, transparency, heterogeneity, distributed computing systems are becoming increasingly popular \cite{DBLP:books/daglib/0017159,DBLP:books/mk/Lynch96}. 

% The Cluster Computing is the most prevalent and fundamental type of distributed computing system \cite{DBLP:journals/computing/SteenT16}. In which, the underlying hardware consists of a collection of similar workstations or PCs, closely connected by means of a high-speed network. A cluster is composed of mainly four components starting from local storage, to distributed storage, communication layer, and, finally, the computing module \cite{DBLP:journals/ftdb/YanBTD17}.

% The PRAM (Parallel Random Access Machine) is also a commonly used parallel computing model. This model assumes the presence of an infinitely large shared memory and multiple processors with similar functionalities. They are capable of performing arithmetic and logical operations as well as data exchange.

The effectiveness and efficiency of distributed computing systems depend on their architecture. The distributed computing architecture defines the organization of data and tasks within the system, the patterns of communication between units, and the system's response mechanisms to failures, which mainly include the following categories:

\noindent\underline{\textit{Master-Worker Architecture.}} The Master-Worker architecture, also known as the Master-Slave architecture, is the most common type of architecture in distributed systems \cite{DBLP:journals/csur/BouhenniYNK21}. The Master serves as the central component of a distributed system, with key responsibilities such as task and resource allocation, as well as data synchronization. On the other hand, the Worker carries out the assigned tasks and provides regular progress updates to the Master. 
MapReduce \cite{DBLP:conf/osdi/DeanG04}, developed by Google, is one of the most popular programming models that utilizes the Master-Worker architecture, and Hadoop \cite{white2012hadoop} is the most well-known open-source distributed computing framework based on Mapreduce. The MapReduce calculation process consists of two stages: Map and Reduce. During the Map stage, data is broken down into key-value pairs and then distributed to different computers for processing. During the Reduce stage, all calculation results are combined and summarized. 
Spark \cite{DBLP:conf/hotcloud/ZahariaCFSS10} is also an open-source, Master-Worker based distributed computing framework. Compared to Hadoop, Spark has more efficient performance of mass data processing due to its RDD memory computing model \cite{DBLP:journals/tjs/HuangQWC20}. 

% \textbf{Three-Tier Architecture.}

\noindent\underline{\textit{Peer-to-Peer.}} The Peer-to-Peer (P2P) architecture is also a popular choice for distributed systems. Unlike the Master-Worker architecture, P2P does not require central servers to coordinate and process data, but instead allows units to communicate and exchange data directly. In the P2P architecture, each unit, or peer, is equal and can both provide and obtain resources from other nodes. There are already many distributed computing systems \cite{DBLP:journals/concurrency/Ernst-DesmulierBS08,DBLP:conf/lcn/SkodzikDARTBD11,DBLP:journals/jpdc/CassaviaFIMP18} designed based on P2P architecture.

Besides, The PRAM (Parallel Random Access Machine) is also a commonly used parallel computing model. This model assumes the presence of an infinitely large shared memory and multiple processors with similar functionalities. Although the PRAM model can not be directly applied to distributed environments, it is possible to design distributed parallel algorithms by simulating the interaction between processors and shared memory in the PRAM model and using effective communication protocols and data sharing methods.

\subsection{Distributed Processing for Graph Algorithms}

Although popular distributed computing frameworks such as Hadoop and Spark are already very mature, they are not suitable for processing graph data \cite{DBLP:journals/csur/McCuneWM15,DBLP:journals/csur/BouhenniYNK21}. Some distributed frameworks \cite{cohen2009graph,kang2009pegasus,DBLP:journals/tkde/ShahrivariJ21} attempt to adapt them to process graph algorithms, but their performance is not satisfactory. On one hand, due to the fact that graph data usually is unstructured and highly irregular, it's difficult for graph computation to scale and parallelize \cite{lumsdaine2007challenges}. On the other hand, graph algorithms typically involve iterative computations between vertices, like PageRank and core decomposition, and each vertex requires access to information about its neighboring vertices. 
Hadoop (or MapReduce programming model) does not directly support iterative algorithms, which requires a cleverly designed multi-round Map/Reduce tasks that greatly increases the programming complexity. While Spark support iterative algorithms, it's global caching mechanism saves intermediate data in memory throughout the iterative process, which leads to extremely high memory requirements for a large number of iterations.

To effectively process graph algorithms, the vertex-centric programming model was first proposed by \cite{DBLP:conf/sigmod/MalewiczABDHLC10}. This model employs a local, vertex-oriented perspective of computation and encourages practitioners to "think like a vertex"  \cite{DBLP:journals/csur/McCuneWM15}. In this programming model, programs are expressed as a sequence of iterations, and each vertex can send and receive messages, and can update its own state based on the state of other vertices in each iteration. Compared to traditional distributed computing frameworks, this approach is more flexible, efficient, and capable of expressing a wide range of algorithms \cite{DBLP:conf/sigmod/MalewiczABDHLC10}.

Influenced by this programming model, an increasing number of distributed graph processing frameworks \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/www/YanCLN15,DBLP:journals/pvldb/HanD15,DBLP:conf/osdi/GonzalezLGBG12,DBLP:journals/tpds/YanHLCCWZ18,DBLP:conf/icfp/RuizMS16,DBLP:journals/tkde/WangWQCZZ23,DBLP:conf/sosp/RoyMZ13,DBLP:journals/fgcs/ZhuHLM20,DBLP:journals/pvldb/TianBCTM13} have been proposed. The programming models for distributed graph processing include three layers: Timing, Communication and Execution Model \cite{DBLP:journals/csur/BouhenniYNK21}, as shown in Figure \ref{fig:programming_models}. Each layer provides multiple options for defining how specific tasks are performed by the system. Table \ref{tab:Programming Models of Distributed Graph Processing Framework} provides an overview of the principal distributed graph processing framework along with their programming models.

\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{pic/programming_models.pdf}

\caption{The Programming Models for Distributed Graph Processing}
\label{fig:programming_models}
% \vspace*{-0.5cm}
\end{figure}


% \subsection{Classification of Distributed Graph programming Models}

\subsubsection{Timing}
In distributed graph algorithms, timing refers to sequence in which tasks or operations are executed, which can be synchronous (all nodes operate in a fixed order) or asynchronous (nodes operate independently without waiting for others) \cite{DBLP:journals/csur/McCuneWM15,DBLP:journals/csur/BouhenniYNK21}. Most distributed graph processing frameworks adopt either a synchronous or an asynchronous model, while several adopt a hybrid model.

\noindent\underline{\textit{Synchronous.}}
% In synchronous timing model, vertices (or units) are executed in parallel different iterations, called supersteps. Only when all tasks have completed their work on the current superstep, the next superstep calculation can be started.
% A famous synchronous processing model is Bulk Synchronous Parallel (BSP) \cite{10.1145/79173.79181}, and a lot of distributed graph processing frameworks adopt this model, such as Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}, Giraph\cite{DBLP:journals/pvldb/HanD15}, GPS\cite{DBLP:conf/ssdbm/SalihogluW13}, Pregel+\cite{DBLP:conf/www/YanCLN15}, etc.
In the synchronous model, vertices (or units) operate in parallel across supersteps, with a global synchronization barrier ensuring all vertices (or units) complete a superstep before moving to the next, thus ensuring the consistent of data access. However, this barrier also presents performance trade-offs due to the waiting periods it imposes.
The Bulk Synchronous Parallel (BSP) framework \cite{10.1145/79173.79181} is a well-known example of this model, which has been widely adopted by distributed graph processing systems like Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}, Giraph\cite{DBLP:journals/pvldb/HanD15}, GPS\cite{DBLP:conf/ssdbm/SalihogluW13}, Pregel+\cite{DBLP:conf/www/YanCLN15}, etc.


\noindent\underline{\textit{Asynchronous.}} 
% In the asynchronous timing model, vertices (or other units) do not need to communicate synchronously, and each vertex can independently perform calculations based on the information it receives. Compared to the synchronous model, the asynchronous model has higher efficiency but relatively greater programming complexity. Some distributed graph processing frameworks \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/osdi/GonzalezLGBG12} adopt this model.
The asynchronous model allows for a more flexible execution where vertices (or units) do not wait for each other and operate independently based on the information available to them at any given time. This approach has greater efficiency, while increases the complexity of algorithms for ensuring the correctness. It is employed by some distributed graph processing frameworks \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/cidr/WangXDG13,DBLP:conf/eurosys/ChenLZYYC18,DBLP:conf/icde/WangGHYH19}. 

\noindent\underline{\textit{Hybrid.}} 
% Both synchronous and asynchronous models have their own advantages and disadvantages. The Hybrid timing model combines synchronous and asynchronous models to balance efficiency and programming complexity in processing distributed graph algorithms. Some distributed graph processing frameworks \cite{DBLP:conf/cidr/WangXDG13,DBLP:journals/corr/ChenBLGSP17} use a mix of synchronous and asynchronous iterations within each superstep, while other frameworks \cite{DBLP:conf/ppopp/XieCGZC15} adaptively switch between the two models to improve performance.
The hybrid model combines elements of both synchronous and asynchronous timing. It aims to balance between the operational efficiency of asynchronous execution and the robustness and data consistency of the synchronous method. This can be implemented in various ways, such as mixing synchronous and asynchronous operations within the same superstep in some frameworks \cite{DBLP:conf/cidr/WangXDG13,DBLP:journals/corr/ChenBLGSP17}, or by adaptively switching between the two modes to optimize performance as observed in others \cite{DBLP:conf/ppopp/XieCGZC15}.

\subsubsection{Communication} Communication in a distributed system refers to the method of message exchange between different units. There are main two communication models: message passing and shared memory.

\noindent\underline{\textit{Message Passing.}}
% In the message passing model, the communication between different vertices (or units) is by sending and receiving messages directly or via message queues, providing high flexibility but requiring complex message management. This model is widely used in distributed systems, such as
% Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}, 
% Giraph\cite{DBLP:journals/pvldb/HanD15}, 
% GPS\cite{DBLP:conf/ssdbm/SalihogluW13}, 
% Giraph++\cite{DBLP:journals/pvldb/TianBCTM13} and 
% Pregel+\cite{DBLP:conf/www/YanCLN15}.
In the message passing model, the communication between different vertices (or units) is by sending and receiving messages directly or via message queues. Its main advantage is the flexibility it offers, which can enhance the scalability of the algorithm. But it increases the complexity of handling message synchronization and ensuring message integrity, requiring some message management strategies. The message passing paradigm is prevalent in distributed graph processing frameworks such as Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}, 
Giraph \cite{DBLP:journals/pvldb/HanD15}, 
GPS \cite{DBLP:conf/ssdbm/SalihogluW13}, 
Giraph++ \cite{DBLP:journals/pvldb/TianBCTM13}, 
Pregel+ \cite{DBLP:conf/www/YanCLN15}, etc., 
which exemplify its widespread adoption in distributed systems.

\noindent\underline{\textit{Shared Memory.}} 
% The shared memory model allows all units to share the same memory space and perform operations there. While simpler, this model requires careful consideration of concurrency control and synchronization issues. GraphLab\cite{DBLP:journals/pvldb/LowGKBGH12} and  PowerGraph\cite{DBLP:conf/osdi/GonzalezLGBG12} employ this model.
In the shared memory model, the data in an unit is exposed as shared variables and it can be directly read or be modiﬁed by any vertices or programs. The frameworks using this model can bypass the memory and processing overhead associated with message passing. It simplifies data access, while presents challenges of ensuring consistency in distributed environments. Implementations of the shared memory model can be seen in frameworks like PowerGraph \cite{DBLP:conf/osdi/GonzalezLGBG12}, Trinity \cite{DBLP:conf/sigmod/ShaoWL13}, BENU \cite{DBLP:conf/icde/WangGHYH19}, WolfGraph \cite{DBLP:journals/fgcs/ZhuHLM20}, etc.

\subsubsection{Execution Model} 

% The execution model is mainly used to define how distributed computing tasks are executed, determining how tasks collaborate on multiple nodes to achieve efficient distributed graph computation. It includes Vertex-Centric, Edge-Centric, and Subgraph-Centric models. 
% The popular Gather-Apply-Scatter (GAS) programming model \cite{DBLP:conf/ppopp/XieCGZC15} divides vertex operations into three steps: Gather, Apply, and Scatter, which can better handle calculation/communication imbalances. Therefore, in this paper, it is categorized as Vertex-Centric. 
% Note that there are other execution models, such as Path-Centric \cite{DBLP:journals/tpds/YuanXLJ16}, with a narrow application scope that are not included in this paper's execution model classification.

In the field of distributed computing, the execution model defines the strategy for task execution across multiple vertices, which is a pivotal factor in achieving efficient processing. There are three prevalent models: Vertex-Centric, Edge-Centric, and Subgraph-Centric, each with its unique approach and suited for different kinds of graph processing tasks.

\noindent\underline{\textit{Vertex-Centric.}} The Vertex-Centric model is the most popular and widely applied execution model, originally introduced in Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}. It is based on a programming abstraction called "thinking like a vertex" (TLAV), where graph processing is done from the perspective of individual vertices. Programmers manipulate each vertex, sending and receiving messages from neighboring vertices during program execution.
Another famous programming model, Gather-Apply-Scatter (GAS) \cite{DBLP:conf/ppopp/XieCGZC15}, also adopts Vertex-Centric execution model, which further refines the process by dividing operations in a vertex into three distinct steps (Gather, Apply, and Scatter) to address communication imbalances.
The simplicity and locality of computation make the Vertex-Centric model a preferred choice for handling complex graph computations in frameworks such as PowerGraph\cite{DBLP:conf/osdi/GonzalezLGBG12}, GPS\cite{DBLP:conf/ssdbm/SalihogluW13}, GraphHP\cite{DBLP:journals/corr/ChenBLGSP17}, etc.
% This model divides vertex operations into three steps: Gather, Apply, and Scatter, which can better handle calculation/communication imbalances.

% The Vertex-Centric model is vertex-based, which make it simple to comprehend and execute. This model only requires each vertex to consider the information of its connected neighbors, rather than the entire graph, which significantly reduces the complexity of designing distributed graph algorithms. As a result, many distributed graph processing frameworks, including
% PowerGraph\cite{DBLP:conf/osdi/GonzalezLGBG12}, 
% GPS\cite{DBLP:conf/ssdbm/SalihogluW13}, 
% GRACE\cite{DBLP:conf/cidr/WangXDG13}, 
% GraphHP\cite{DBLP:journals/corr/ChenBLGSP17},
% Pregel+\cite{DBLP:conf/www/YanCLN15}, 
% Giraph\cite{DBLP:journals/pvldb/HanD15}, 
% PowerSwitch \cite{DBLP:conf/ppopp/XieCGZC15},
% s6raph\cite{DBLP:conf/icfp/RuizMS16},
% GraphD\cite{DBLP:journals/tpds/YanHLCCWZ18},
% ScaleG\cite{DBLP:journals/tkde/WangWQCZZ23},
% adopt this model due to its advantages.


\noindent\underline{\textit{Edge-Centric.}} 
The Edge-Centric model, initially introduced by X-Stream \cite{DBLP:conf/sosp/RoyMZ13}, shifts focus from vertices to edges, which independently manage their states and communicate directly with each other. 

This approach provides better performance for non-uniform graphs, especially those with power-law distributions, by streamlining interactions among edges and bypassing the random memory accesses associated with vertices \cite{DBLP:journals/csur/HeidariSCB18}. While the Edge-Centric model tends to be more complex to program, it offers enhanced performance for algorithms that require pre-processing of sorting edge lists, like BFS \cite{DBLP:journals/fgcs/ZhuHLM20, DBLP:conf/sosp/RoyMZ13}. Moreover, for large-scale graphs where the edge set vastly exceeds the vertex set, this model demonstrates superior performance due to its eliminating random memory accesses to edges \cite{DBLP:conf/cf/ZhouKZP18}. In addition to X-Stream, WolfGraph \cite{DBLP:journals/fgcs/ZhuHLM20} also adopts this execution model.


% First proposed in X-Stream \cite{DBLP:conf/sosp/RoyMZ13}, the Edge-Centric model pivots the computational workload to the edges of the graph, iterating over them for processing. In this model, edges manage their own state and communicate with adjacent edges. In addition to X-Stream, WolfGraph \cite{DBLP:journals/fgcs/ZhuHLM20} also adopts this execution model.
% % Although being harder to implement than the Vertex-Centric model, the Edge-Centric model can offer better performance in certain algorithms. 

% The Edge-Centric model, while providing better performance for graph processing, particularly for non-uniform graphs like those with power-law distributions, incurs higher complexity in programming \cite{DBLP:journals/csur/HeidariSCB18}. It performs better in algorithms that require pre-processing of sorting edge lists, like BFS \cite{DBLP:journals/fgcs/ZhuHLM20, DBLP:conf/sosp/RoyMZ13}.  
% Besides, the Edge-Centric model outperforms the Vertex-Centric approach for large-scale graphs by eliminating random memory accesses to edges, leading to better performance \cite{DBLP:conf/cf/ZhouKZP18}.


% The Edge-Centric model (first proposed in \cite{DBLP:conf/sosp/RoyMZ13}) is an execution model where the edge is the primary unit of computation and the program iterates over edges of the graph. In this model, edges can communicate with their neighboring edges by sending and receiving messages \cite{DBLP:journals/csur/BouhenniYNK21}.

% X-Stream\cite{DBLP:conf/sosp/RoyMZ13} is the first distributed graph processing framework using Edge-Centric model in order to cope with the challenge of the lack of access locality when traversing edges. In addition to X-Stream, \cite{DBLP:conf/cf/ZhouKZP18} and WolfGraph\cite{DBLP:journals/fgcs/ZhuHLM20} are also use this execution model.

% Algorithm Edge-Centric model is more difficult to implement than Vertex-Centric, it has been empirically shown that frameworks which use Edge-Centric model can perform more efficiency \cite{DBLP:journals/csur/HeidariSCB18}. The advantage of Edge-Centric model is that it traverses the edges in a streaming fashion, so it does not require any pre-processing of the data \cite{DBLP:conf/cf/ZhouKZP18}.

\noindent\underline{\textit{Subgraph-Centric.}} The Subgraph-Centric model, also known as Block-Centric model, is based on a programming abstraction called "think like a graph" \cite{DBLP:journals/pvldb/TianBCTM13}. This model focuses on the entire subgraph rather than vertices or edges, and the message exchange occurs on the subgraph in each iteration \cite{DBLP:journals/tpds/ZhangJHLYY23}. Communication between vertices within a subgraph does not delay until the next superstep, but is executed immediately \cite{DBLP:journals/csur/BouhenniYNK21}.

Compared to other models, the Subgraph-Centric model involves less communication, making it more suitable for graph analysis tasks where vertices need to frequently communicate with their neighbors, such as social network analysis, local clustering coefficient calculation, and anomaly detection \cite{DBLP:conf/sigmod/QuamarD16}. However, it is not suitable for power-law graphs \cite{DBLP:conf/ppopp/XieCGZC15}, and its performance relies on sophisticated graph partitioning and preprocessing techniques \cite{DBLP:journals/tpds/ZhangJHLYY23}.  
Distributed graph processing frameworks which adopt Subgraph-Centric model include 
Giraph++\cite{DBLP:journals/pvldb/TianBCTM13}, GoFFish\cite{DBLP:conf/europar/SimmhanKWNRRP14}, Blogel\cite{DBLP:journals/pvldb/YanCLN14}, etc.


% GoFFish\cite{DBLP:conf/europar/SimmhanKWNRRP14},
% Blogel\cite{DBLP:journals/pvldb/YanCLN14},
% Nscale\cite{DBLP:journals/vldb/QuamarDL16},
% NScaleSpark\cite{DBLP:conf/sigmod/QuamarD16},
% DRONE\cite{DBLP:journals/tpds/ZhangJHLYY23},
% G-thinker\cite{DBLP:journals/vldb/YanGKOKL22},
% BENU\cite{DBLP:conf/icde/WangGHYH19},
% G-Miner\cite{DBLP:conf/eurosys/ChenLZYYC18}, etc.




==> section/sec2_Distributed_Graph_Processing2.tex <==
In the real world, there is an amount of data, including social networks, road networks, and text data, requires efficient processing and analysis. However, the limited performance and memory capacity of single machines often lead to inefficiencies, especially in graph data processing. Therefore, dividing and deploying data across multiple machines and distributed computing present a prevalent and effective solution.
General distributed frameworks, such as Hadoop and Spark which all adapt MapReduce programming model, are not ideally suited for processing graph data, since graph data is typically unstructured and highly irregular, making computation difficult to scale and parallelize. Most graph algorithms, like PageRank and k-core decomposition, involve iterative computations among vertices, where each vertex needs access to information about its neighboring vertices.
However, Hadoop does not directly support iterative algorithms which are essential in graph processing, leading to the need for complex multi-round Map/Reduce tasks. Spark, while supporting iterative algorithms, faces challenges with its global caching mechanism, especially for large-scale data, resulting in high memory requirements.

To effectively process graph data in distributed environments, a variety of distributed graph programming models have been proposed. These models allow the definition of graph data structures and enable the efficient expression of complex graph algorithms.
In this section, we discuss how distributed graph processing models express complex graph algorithms in a distributed environment, using the most popular TLAV framework (think like a vertex) as an example. We also provide an overview of various other distributed graph processing frameworks and categorize their programming models, discussing their unique features and contributions to optimizing graph processing challenges.

% \subsection{TLAV Framework} 
\subsection{General-Purpose Distributed Processing Frameworks} 
The TLAV framework (also called Vertex-Centric) emphasize a localized, vertex-oriented perspective, i.e., all computation is focused on the vertices of a graph. In this framework, a user-defined program is iteratively executed over the vertices of a graph. Each vertex processes data based on its local state, which includes information from adjacent vertices or incoming edges \cite{DBLP:journals/csur/McCuneWM15}. This processing approach provides a natural way to express and compute many iterative graph algorithms.

In TLAV framework, the computation on the graph is divided into a series of synchronized iterations, each of which is called a superstep. During a single superstep, each vertex executes a user-defined function in parallel. This function typically processes data based on the vertex's current state and the messages it received from other vertices \cite{DBLP:journals/tkde/KalavriVH18}. A global synchronization barrier is used to ensure all vertices complete a superstep before moving to the next, thus ensuring the consistent of data access. However, this barrier also presents performance trade-offs due to the waiting periods it imposes.
Besides, vertices communicate with each other usually through sending and receiving messages directly. Messages sent during a superstep are delivered in batches at the beginning of the next superstep. Its main advantage is the flexibility it offers, which can enhance the scalability of the algorithm. But it increases the complexity of handling message synchronization and ensuring message integrity, and requires some message management strategies.

The vertex functions in TLAV framework encompasses three primary approaches: one-phase model, Scatter-Gather model and Gather-Apply-Scatter (GAS) model, each with its own method of handling vertex operations.
The one-phase model, exemplified by Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}, involves a single function for processing input, computing new vertex values, updating and sending out new values. This model is straightforward but limits flexibility, which may causes challenges of load balancing and iteration inefficiency. The Scatter-Gather model separates the process into scattering vertex values to neighbors and gathering inputs for updates, as seen. Finally, the Gather-Apply-Scatter (GAS) model, introduced by PowerGraph \cite{DBLP:conf/osdi/GonzalezLGBG12}, involves aggregating input data, updating vertex values, and then propagating these updates, which is particularly effective for processing power-law graphs.

% The first programming model adapting TLAV framework is Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}. Influenced by it, an increasing number of distributed graph processing frameworks \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/www/YanCLN15,DBLP:journals/pvldb/HanD15,DBLP:conf/osdi/GonzalezLGBG12,DBLP:journals/tpds/YanHLCCWZ18,DBLP:conf/icfp/RuizMS16,DBLP:journals/tkde/WangWQCZZ23,DBLP:conf/sosp/RoyMZ13,DBLP:journals/fgcs/ZhuHLM20,DBLP:journals/pvldb/TianBCTM13} have been proposed. There are a lot of variants for optimizing distributed computing. Some programming models like GraphLab \cite{DBLP:journals/pvldb/LowGKBGH12} and Trinity \cite{DBLP:conf/sigmod/ShaoWL13} allow asynchronous execution to enhance parallelism. The Gather-Sum-Apply-Scatter (GAS) model, introduced by PowerGraph \cite{DBLP:conf/osdi/GonzalezLGBG12}, decomposes processing in vertices into four distinct phases to handle computational imbalances in graphs, particularly in those with vertices of varying degrees. 

% \subsection{Classification of Programming Models}

\subsection{Distributed Graph Processing Frameworks}

The TLAV framework is applicable to an amount of graph algorithms, allowing programmers to use design logic similar to that of single-machine algorithms for designing distributed algorithms. However, this model is not suitable for all graph algorithms. 
% For non-iterative algorithms that do not require multiple rounds of iterative state updates, this superstep-based iterative method may lead to unnecessary computational and communication overhead, thereby reducing the overall efficiency of the algorithm. 
Due to it requires computation to be expressed from the perspective of a single vertex, all non-local (more than one hop) state updates must be communicated through message passing. For algorithms, like triangle counting, that require global or multi-hop neighbor information, such limitations make the implementation of the algorithm complex and inefficient.

In addition to TLAV frameworks, there are many other distributed graph processing frameworks designed to address the challenges of various distributed graph algorithms. In this paper, we have surveyed over 20 distributed graph processing frameworks and categorized their programming models into three layers: Timing, Communication and Execution Model. Table \ref{tab:Programming Models of Distributed Graph Processing Framework} provides an overview of those frameworks along with their programming models.

\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{pic/programming_models.pdf}

\caption{The Programming Models for Distributed Graph Processing}
\label{fig:programming_models}
% \vspace*{-0.5cm}
\end{figure}

\begin{table}[h]
\caption{Programming Models of Distributed Graph Processing Framework}
\label{tab:Programming Models of Distributed Graph Processing Framework}
\begin{tabular}{l|rrrr}
\hline
\textbf{Framework}   & \textbf{Timing}               & \textbf{Communication}  & \textbf{Execution Model}                      & \textbf{Year}                     \\ \hline
Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}      & Synchronous          & Message Passing    & Vertex-Centric                       & 2010                     \\
GraphLab \cite{DBLP:journals/pvldb/LowGKBGH12}   & Asynchronous         & Message Passing      & Vertex-Centric                       & 2012                     \\
PowerGraph \cite{DBLP:conf/osdi/GonzalezLGBG12} & Hybrid                  & Shared Memory                     & Vertex-Centric                       & 2012                     \\
GPS \cite{DBLP:conf/ssdbm/SalihogluW13}        &  Synchronous                    & Message Passing                     & Vertex-Centric                       & 2013                     \\
Giraph++ \cite{DBLP:journals/pvldb/TianBCTM13}   & Hybrid                    & Message Passing                     & Subgraph-Centric                     & 2013                     \\
GRACE \cite{DBLP:conf/cidr/WangXDG13}      & Hybrid               & Message Passing      & Vertex-Centric                       & 2013                     \\
Trinity \cite{DBLP:conf/sigmod/ShaoWL13}      & Asynchronous               & Shared Memory      & Vertex-Centric                       & 2013                     \\
GoFFish \cite{DBLP:conf/europar/SimmhanKWNRRP14}    &  Synchronous                    & Both                       & Subgraph-Centric                     & 2014                     \\
Blogel \cite{DBLP:journals/pvldb/YanCLN14}     & Synchronous                     & Message Passing                      & Subgraph-Centric                     & 2014                     \\
Giraph \cite{DBLP:journals/pvldb/HanD15}     & Synchronous          & Message Passing      & Vertex-Centric                       & 2015                     \\
Pregel+ \cite{DBLP:conf/www/YanCLN15}    &  Synchronous                    & Message Passing                     & Vertex-Centric                       & 2015                     \\
PowerSwitch \cite{DBLP:conf/ppopp/XieCGZC15} & Hybrid               & Message Passing    & Vertex-Centric                       & 2015                     \\
s6raph \cite{DBLP:conf/icfp/RuizMS16}     & Synchronous                     &  Message Passing                       & Vertex-Centric                       & 2016                     \\
Nscale \cite{DBLP:journals/vldb/QuamarDL16}     &  Synchronous                    & Message Passing                      & Subgraph-Centric                     & 2016                     \\
NScaleSpark \cite{DBLP:conf/sigmod/QuamarD16} & Synchronous & Message Passing  & Subgraph-Centric & \multicolumn{1}{l}{2016} \\

GraphHP \cite{DBLP:journals/corr/ChenBLGSP17}    & Synchronous               & Message Passing      & Vertex-Centric                       & 2017                     \\
GraphD \cite{DBLP:journals/tpds/YanHLCCWZ18}     & Synchronous                     & Message Passing                     & Vertex-Centric                       & 2018                     \\
X-Stream \cite{DBLP:conf/sosp/RoyMZ13}  &   Synchronous                   &   Message Passing                     & Edge-Centric                         & 2018                     \\
G-Miner \cite{DBLP:conf/eurosys/ChenLZYYC18}     & Asynchronous                    & Message Passing                     & Subgraph-Centric                     & 2018                     \\
BENU \cite{DBLP:conf/icde/WangGHYH19}      & Asynchronous                     &  Shared Memory                    & Subgraph-Centric                     & 2019                     \\
WolfGraph \cite{DBLP:journals/fgcs/ZhuHLM20}  &  Synchronous                    & Shared Memory                     & Edge-Centric                         & 2020                     \\
% G-thinker \cite{DBLP:journals/vldb/YanGKOKL22}   & Synchronous?                     &  Shared Memory?                    & Subgraph-Centric                     & 2022                     \\
DRONE \cite{DBLP:journals/tpds/ZhangJHLYY23}       & Synchronous                     &Message Passing                      & Subgraph-Centric                     & 2023                     \\
ScaleG \cite{DBLP:journals/tkde/WangWQCZZ23}     & Synchronous                     & Message Passing                     & Vertex-Centric                       & 2023                     \\
 \hline
\end{tabular}
\end{table}

% \underline{\textit{Timing.}} Timing, crucial in task execution order, is predominantly synchronous in distributed frameworks, offering ease of programming and suitability for iterative algorithms \cite{DBLP:conf/sigmod/MalewiczABDHLC10,DBLP:conf/ssdbm/SalihogluW13}. However, some frameworks adopt asynchronous or hybrid models for more flexible and efficient execution, albeit increasing algorithm complexity \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/cidr/WangXDG13,DBLP:conf/eurosys/ChenLZYYC18,DBLP:conf/icde/WangGHYH19}.

% \underline{\textit{Communication.}} Communication methods in distributed graph processing primarily involve message passing, offering scalability and flexibility, yet posing challenges in frequent neighbor interactions or global information requirements. Alternatively, shared memory allows direct data access, simplifying data handling but complicating consistency maintenance in distributed settings.


\underline{\textit{Timing.}} Timing refers to sequence in which tasks or operations are executed, which can be synchronous or asynchronous. Synchronous model is the main choice for most distributed frameworks \cite{DBLP:conf/sigmod/MalewiczABDHLC10,DBLP:conf/ssdbm/SalihogluW13,}, since it is easy for programming and suits to most algorithms, particularly those based on iterative computations. While some frameworks \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/cidr/WangXDG13,DBLP:conf/eurosys/ChenLZYYC18,DBLP:conf/icde/WangGHYH19,} choose asynchronous or hybrid model that allows a more flexible execution where vertices do not wait for each other and operate independently based on their received information.
This approach has greater efficiency, while increases the complexity of algorithms for ensuring the correctness. 

\underline{\textit{Communication.}} Communication in a distributed system refers to the method of message exchange between different units or vertices, main includes message passing and shared memory. Message passing is the main communication approach in distributed graph processing. Its main advantage is the flexibility it offers, which can enhance the scalability of the algorithm. However, for algorithms that require frequent exchanges of information with neighbors or need global information, this may pose the challenge communication overhead. The shared memory method lets data expose as shared variables that can be directly read or be modified by any vertices or programs. It simplifies data access, while presents challenges of ensuring consistency in distributed environments.

% \underline{\textit{Execution Model.}} The execution model defines the strategy for task execution across multiple vertices, which is a pivotal factor in achieving efficient processing. In addition to the Vertex-Centric model in TLAV frameworks, there are also other models, Edge-Centric and Subgraph-Centric.

% The Edge-Centric model, initially introduced by X-Stream \cite{DBLP:conf/sosp/RoyMZ13}, shifts focus from vertices to edges, which independently manage their states and communicate directly with each other. 
% This approach provides better performance for non-uniform graphs, especially those with power-law distributions, by streamlining interactions among edges and bypassing the random memory accesses associated with vertices \cite{DBLP:journals/csur/HeidariSCB18}. While the Edge-Centric model tends to be more complex to program, it offers enhanced performance for algorithms that require pre-processing of sorting edge lists, like BFS \cite{DBLP:journals/fgcs/ZhuHLM20, DBLP:conf/sosp/RoyMZ13}. Moreover, for large-scale graphs where the edge set vastly exceeds the vertex set, this model demonstrates superior performance due to its eliminating random memory accesses to edges \cite{DBLP:conf/cf/ZhouKZP18}. In addition to X-Stream, WolfGraph \cite{DBLP:journals/fgcs/ZhuHLM20} also adopts this execution model.

% The Subgraph-Centric model, is based on a programming abstraction called "think like a graph" \cite{DBLP:journals/pvldb/TianBCTM13}. This model focuses on the entire subgraph rather than vertices or edges, and the message exchange occurs on the subgraph in each iteration \cite{DBLP:journals/tpds/ZhangJHLYY23}. Communication between vertices within a subgraph does not delay until the next superstep, but is executed immediately \cite{DBLP:journals/csur/BouhenniYNK21}.
% Compared to other models, the Subgraph-Centric model involves less communication, making it more suitable for graph analysis tasks where vertices need to frequently communicate with their neighbors, such as social network analysis, local clustering coefficient calculation, and anomaly detection \cite{DBLP:conf/sigmod/QuamarD16}. However, it is not suitable for power-law graphs \cite{DBLP:conf/ppopp/XieCGZC15}, and its performance relies on sophisticated graph partitioning and preprocessing techniques \cite{DBLP:journals/tpds/ZhangJHLYY23}.  
% Distributed graph processing frameworks which adopt Subgraph-Centric model include 
% Giraph++\cite{DBLP:journals/pvldb/TianBCTM13}, GoFFish\cite{DBLP:conf/europar/SimmhanKWNRRP14}, Blogel\cite{DBLP:journals/pvldb/YanCLN14}, etc.

\underline{\textit{Execution Model.}} The execution model defines the strategy for task execution across multiple vertices, which is a pivotal factor in achieving efficient processing. Beyond the Vertex-Centric model in TLAV frameworks, the Edge-Centric and Subgraph-Centric models offer enhancements in different aspects. The Edge-Centric model, pioneered by X-Stream \cite{DBLP:conf/sosp/RoyMZ13}, focuses on edges rather than vertices. This approach provides better performance for non-uniform graphs, especially those with power-law distributions, by streamlining interactions among edges and bypassing the random memory accesses associated with vertices \cite{DBLP:journals/csur/HeidariSCB18}. While the Edge-Centric model tends to be more complex to program, it offers enhanced performance for algorithms that require pre-processing of sorting edge lists, like BFS \cite{DBLP:journals/fgcs/ZhuHLM20, DBLP:conf/sosp/RoyMZ13}. 

The Subgraph-Centric model, encapsulated by the "think like a graph" abstraction, concentrates on entire subgraphs. This model minimizes communication overhead, making it ideal for tasks where frequent vertex interaction is crucial, such as in social network analysis. However, it is less effective for power-law graphs and relies heavily on advanced graph partitioning techniques \cite{DBLP:journals/tpds/ZhangJHLYY23, DBLP:journals/csur/BouhenniYNK21, DBLP:conf/sigmod/QuamarD16, DBLP:conf/ppopp/XieCGZC15}. Frameworks like Giraph++, GoFFish, and Blogel adapt this model \cite{DBLP:journals/pvldb/TianBCTM13, DBLP:conf/europar/SimmhanKWNRRP14, DBLP:journals/pvldb/YanCLN14}.


==> section/sec2_Distributed_Graph_Processing3.tex <==

% In the real world, there is an amount of graph data, including social networks, road networks, and web networks, requires efficient processing and analysis. However, the limited performance and memory capacity of single machines often lead to inefficiencies, especially in graph data processing. Therefore, dividing and deploying data across multiple machines and distributed computing present a prevalent and effective solution. Building upon this necessity, in this section, we delve into the distributed graph processing infrastructure critical for implementing distributed graph algorithms. We explore various tools and frameworks, starting from fundamental distributed programming interfaces (section 2.1), general-purpose distributed processing frameworks (section 2.2) to more complex distributed processing frameworks designed for graph algorithms (section 2.3).
% This comprehensive review not only showcases the current distributed graph processing infrastructure but also sets the stage for the following research of the challenges within distributed environments and the state-of-the-art distributed graph algorithms.

Dis

Applying algorithms on distributed systems often involves many complex non-algorithmic operations, such as data partitioning, communication across various machines and data synchronization. Abstracting these into unified interfaces allows programmers to concentrate on algorithm design rather than low-level details of distributed computation.
In this section, we delve into the distributed graph processing infrastructure, starting from fundamental distributed programming interfaces (section 2.1), general-purpose distributed processing frameworks (section 2.2) to more complex distributed processing frameworks designed for graph algorithms (section 2.3).
% This comprehensive review not only showcases the current distributed graph processing infrastructure but also sets the stage for the following research of the challenges within distributed environments and the state-of-the-art distributed graph algorithms.



% \subsection{Foundational Distributed Programming Interfaces}
\subsection{Distributed Programming Interface}

The Message Passing Interface (MPI) \cite{forum1994mpi} is a message passing standard designed for developing parallel algorithms in distributed systems. It provides communication and synchronization between processes through message passing. 
% One of the advantages of MPI is its portability, as its implementation (like OpenMPI \cite{graham2006open} or MPICH \cite{gropp1996high}) provides directly callable APIs for nearly all major programming languages, including C, C++, Fortran, Python, and Java. 
One of the advantages of MPI is its portability, as its implementation (like OpenMPI \cite{graham2006open} or MPICH \cite{gropp1996high}) provides directly callable APIs capitalizing with nearly all major programming languages.
Furthermore, MPI offers a range of advanced functionalities such as inter-cluster communication, one-sided communication, custom data types, and process management. These features let MPI become a popular choice for underlying communication in many advanced distributed frameworks. 

Partitioned Global Address Space (PGAS) is another widely-used programming model for distributed computing. Unlike MPI using the explicit message-passing, PGAS provides a global memory address space abstraction, i.e., it allows programmers to directly access remote memory, while the underlying message-passing is automatically managed by PGAS. This feature offers advantages in usability and programming simplicity, but it also loses the flexibility of controlling communication details. There are several popular implementations of PGAS, such as OpenSHMEM \cite{chapman2010introducing}, PCJ \cite{nowicki2012parallel}, X10 \cite{charles2005x10} and Chapel \cite{chapel2017chapel}.


% In distributed systems, data is spread across multiple computing units. Designing algorithms for such environments is not straightforward due to the need for efficient and reliable communication between these units. This requirement led to the development of the Message Passing Interface (MPI), a widely used communication standard for passing messages between different units in a distributed environment. It provides various API and is designed to meet the complex communication needs of distributed computing, where extensive data exchange and precise synchronization are often necessary. 

% For the design of distributed graph algorithms, MPI plays a very important role. 
% Graph algorithms, by their nature, involve complex relationships and interdependencies among vertices. Tasks such as triangle counting, finding shortest paths, or calculating centrality, which are already computationally intensive on a single machine, become even more complex in a distributed environment. MPI not only facilitates data communication but also offers effective ways to coordinate and synchronize actions across different units, ensuring the accuracy and efficiency of the algorithms.


% For the distributed graph algorithms, the role of MPI is crucial. It not only facilitates data communication but also offers effective ways to coordinate and synchronize actions across different units, ensuring the accuracy and efficiency of the algorithms.

% In the quest to unravel the complexities of distributed graph algorithms, the bedrock lies in the selection of an appropriate programming model. Each model presents its own strategy for decomposing complex graph problems into manageable computations that can be processed across multiple computing nodes. This section introduces four pivotal models that have shaped the field.

% \underline{\textit{MPI.}} MPI (Message Passing Interface) is the cornerstone of in the realm of parallel computing across distributed memory systems. It allows multiple processors to communicate with one another using message-passing techniques. MPI's prowess is anchored in its flexible communication mechanisms, which enable precise data distribution and flow control—critical for the fine-grained synchronization and load balancing inherent in graph algorithms.

% \underline{\textit{OpenMP.}} Contrasting MPI's distributed memory paradigm, OpenMP (Open Multi-Processing) offers a shared memory parallel programming approach. Leveraging multi-threaded execution on multi-core processors, OpenMP facilitates the rapid implementation of parallel graph algorithms, such as dynamic programming and traversal techniques.

% \underline{\textit{BSP.}} The BSP (Bulk Synchronous Parallel) model presents that the computation on the graph is divided into a series of synchronized iterations, each of which is called a superstep. During a single superstep, each vertex executes a user-defined function in parallel. This function typically processes data based on the vertex's current state and the messages it received from other vertices \cite{DBLP:journals/tkde/KalavriVH18}. A global synchronization barrier is used to ensure all vertices complete a superstep before moving to the next, thus ensuring the consistent of data access. However, this barrier also presents performance trade-offs due to the waiting periods it imposes.

% \underline{\textit{MapReduce.}} MapReduce \cite{DBLP:conf/osdi/DeanG04}, developed by Google, is one of the most popular programming models that utilizes the Master-Worker architecture. The MapReduce calculation process consists of two stages: Map and Reduce. During the Map stage, data is broken down into key-value pairs and then distributed to different computers for processing. During the Reduce stage, all calculation results are combined and summarized. This model abstracts the complexity of distributed computing, allowing developers to focus on the mapping and reduction functions of their algorithms, while it does not directly support iterative algorithms which are essential in graph processing, leading to the need for complex multi-round Map/Reduce tasks.


\subsection{General-Purpose Distributed Processing Frameworks}

% In the previous section, we discussed MPI and its importance in designing distributed graph algorithms. While MPI is a powerful tool and offers considerable flexibility in programming, its utilization comes with inherent complexities. This is particularly evident when dealing with complex algorithms, where programming and debugging of MPI-based solutions can pose significant challenges. Those led to a demand for more easy-used and feature-rich distributed processing frameworks.

Distributed programming interfaces discussed earlier provide efficient distributed computing and data communication, while they also bring complexity in programming and debugging. That leads to a demand for more easy-used and feature-rich distributed processing frameworks.

% Apache Hadoop \cite{white2012hadoop} is one of the widely used general-purpose distributed processing frameworks, which adapt MapReduce programming model \cite{DBLP:conf/osdi/DeanG04}. The MapReduce calculation process consists of two stages: Map and Reduce. During the Map stage, data is broken down into key-value pairs and then distributed to different computers for processing, and during the Reduce stage, all calculation results are combined and summarized. Thanks to the MapReduce, Hadoop abstracts the complexity of distributed computing, allowing developers to focus on the mapping and reduction functions of their algorithms. 
% There are many distributed graph algorithms \cite{DBLP:conf/iccnc/GandhiM15,hernandez2016distributed} have already been implemented using this framework. However, Hadoop is not suited for those graph algorithms, like PageRank and k-core decomposition, involving iterative computations among vertices. Each iteration requires reading from and writing to the disk, leading to significant overhead and inefficiency.

MapReduce \cite{DBLP:conf/osdi/DeanG04} is a popular programming model for processing large-scale data in distributed environments, which consists of two stages: Map and Reduce. During the Map stage, data is broken down into key-value pairs and then distributed to different computers for processing, and during the Reduce stage, all calculation results are combined and summarized. Apache Hadoop \cite{white2012hadoop} is an popular open source implementation using MapReduce, which provides a series of software supporting distributed computing. Hadoop abstracts lower-level details of distributed processing, allowing developers to focus on the mapping and reduction functions of their algorithms. 
There are many distributed graph algorithms \cite{DBLP:conf/iccnc/GandhiM15,hernandez2016distributed} have already been implemented using this framework. However, it is not suited for the graph algorithms, like PageRank and k-core decomposition, involving iterative computations among vertices. Each iteration requires reading from and writing to the disk, leading to significant overhead and inefficiency.

Apache Spark \cite{DBLP:conf/hotcloud/ZahariaCFSS10} is another open-source engine allowing distributed computing. Spark provides a more flexible in-memory processing, i.e., allows intermediate results save in memory. This attribute, compared to Hadoop involving disk-heavy operations, make Spark support graph algorithms that need iterative computation. However, this also means that Spark has higher requirements for memory. In environments where resources are limited, this could constrain its performance and scalability, especially processing large-scale graph data.

\subsection{Distributed Graph Processing Frameworks}

Spark and Hadoop generate a large amount of intermediate data within each iteration, this significantly reduces performance when processing graph algorithms that require frequent access to and updates information of vertices. Therefore, a variety of distributed graph programming models are proposed to effectively process graph data in distributed environments. These models allow the definition of graph data structures and enable the efficient expression of complex graph algorithms. Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10} is the first distributed processing framework designed for processing graph data, which use the most popular TLAV (think like a vertex) framework. 
The TLAV framework emphasize a localized, vertex-oriented perspective, i.e., all computation is focused on the vertices of a graph. In this framework, a user-defined program is iteratively executed over the vertices of a graph. Each vertex processes data based on its local state, which includes information from adjacent vertices or incoming edges \cite{DBLP:journals/csur/McCuneWM15}. This processing approach provides a natural way to express and compute many iterative graph algorithms. 

In TLAV framework, the computation on the graph is divided into a series of synchronized iterations, each of which is called a superstep. During a single superstep, each vertex executes a user-defined function in parallel. This function typically processes data based on the vertex's current state and the messages it received from other vertices \cite{DBLP:journals/tkde/KalavriVH18}. A global synchronization barrier is used to ensure all vertices complete a superstep before moving to the next, thus ensuring the consistent of data access. However, this barrier also presents performance trade-offs due to the waiting periods it imposes.
Besides, vertices communicate with each other usually through sending and receiving messages directly. Messages generated during a superstep are delivered in batches at the beginning of the next superstep. Its main advantage is the flexibility it offers, which can enhance the scalability of the algorithm. But it increases the complexity of handling message synchronization and ensuring message integrity, and requires some message management strategies.

However, this model is not suitable for all graph algorithms.
Due to it requires computation to be expressed from the perspective of a single vertex, all non-local (more than one hop) state updates must be communicated through message passing. For algorithms, like triangle counting, that require global or multi-hop neighbor information, such limitations make the implementation of the algorithm complex and inefficient. In addition to TLAV frameworks, there are many other distributed graph processing frameworks designed to address the challenges of various distributed graph algorithms. In this paper, we categorize those programming models into three layers: Timing, Communication and Execution Model. Table \ref{tab:Programming Models of Distributed Graph Processing Framework} provides an overview of those frameworks along with their programming models.

\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth]{pic/programming_models.pdf}

\caption{The Programming Models for Distributed Graph Processing}
\label{fig:programming_models}
% \vspace*{-0.5cm}
\end{figure}

\begin{table}[h]
\caption{Programming Models of Distributed Graph Processing Framework}
\label{tab:Programming Models of Distributed Graph Processing Framework}
\begin{tabular}{l|rrrr}
\hline
\textbf{Framework}   & \textbf{Timing}               & \textbf{Communication}  & \textbf{Execution Model}                      & \textbf{Year}                     \\ \hline
Pregel \cite{DBLP:conf/sigmod/MalewiczABDHLC10}      & Synchronous          & Message Passing    & Vertex-Centric                       & 2010                     \\
GraphLab \cite{DBLP:journals/pvldb/LowGKBGH12}   & Asynchronous         & Message Passing      & Vertex-Centric                       & 2012                     \\
PowerGraph \cite{DBLP:conf/osdi/GonzalezLGBG12} & Hybrid                  & Shared Memory                     & Vertex-Centric                       & 2012                     \\
GPS \cite{DBLP:conf/ssdbm/SalihogluW13}        &  Synchronous                    & Message Passing                     & Vertex-Centric                       & 2013                     \\
Giraph++ \cite{DBLP:journals/pvldb/TianBCTM13}   & Hybrid                    & Message Passing                     & Subgraph-Centric                     & 2013                     \\
GRACE \cite{DBLP:conf/cidr/WangXDG13}      & Hybrid               & Message Passing      & Vertex-Centric                       & 2013                     \\
Trinity \cite{DBLP:conf/sigmod/ShaoWL13}      & Asynchronous               & Shared Memory      & Vertex-Centric                       & 2013                     \\
GoFFish \cite{DBLP:conf/europar/SimmhanKWNRRP14}    &  Synchronous                    & Both                       & Subgraph-Centric                     & 2014                     \\
Blogel \cite{DBLP:journals/pvldb/YanCLN14}     & Synchronous                     & Message Passing                      & Subgraph-Centric                     & 2014                     \\
Giraph \cite{DBLP:journals/pvldb/HanD15}     & Synchronous          & Message Passing      & Vertex-Centric                       & 2015                     \\
Pregel+ \cite{DBLP:conf/www/YanCLN15}    &  Synchronous                    & Message Passing                     & Vertex-Centric                       & 2015                     \\
PowerSwitch \cite{DBLP:conf/ppopp/XieCGZC15} & Hybrid               & Message Passing    & Vertex-Centric                       & 2015                     \\
s6raph \cite{DBLP:conf/icfp/RuizMS16}     & Synchronous                     &  Message Passing                       & Vertex-Centric                       & 2016                     \\
Nscale \cite{DBLP:journals/vldb/QuamarDL16}     &  Synchronous                    & Message Passing                      & Subgraph-Centric                     & 2016                     \\
NScaleSpark \cite{DBLP:conf/sigmod/QuamarD16} & Synchronous & Message Passing  & Subgraph-Centric & \multicolumn{1}{l}{2016} \\

GraphHP \cite{DBLP:journals/corr/ChenBLGSP17}    & Synchronous               & Message Passing      & Vertex-Centric                       & 2017                     \\
GraphD \cite{DBLP:journals/tpds/YanHLCCWZ18}     & Synchronous                     & Message Passing                     & Vertex-Centric                       & 2018                     \\
X-Stream \cite{DBLP:conf/sosp/RoyMZ13}  &   Synchronous                   &   Message Passing                     & Edge-Centric                         & 2018                     \\
G-Miner \cite{DBLP:conf/eurosys/ChenLZYYC18}     & Asynchronous                    & Message Passing                     & Subgraph-Centric                     & 2018                     \\
BENU \cite{DBLP:conf/icde/WangGHYH19}      & Asynchronous                     &  Shared Memory                    & Subgraph-Centric                     & 2019                     \\
WolfGraph \cite{DBLP:journals/fgcs/ZhuHLM20}  &  Synchronous                    & Shared Memory                     & Edge-Centric                         & 2020                     \\
% G-thinker \cite{DBLP:journals/vldb/YanGKOKL22}   & Synchronous?                     &  Shared Memory?                    & Subgraph-Centric                     & 2022                     \\
DRONE \cite{DBLP:journals/tpds/ZhangJHLYY23}       & Synchronous                     &Message Passing                      & Subgraph-Centric                     & 2023                     \\
ScaleG \cite{DBLP:journals/tkde/WangWQCZZ23}     & Synchronous                     & Message Passing                     & Vertex-Centric                       & 2023                     \\
 \hline
\end{tabular}
\end{table}


\underline{\textit{Timing.}} Timing refers to sequence in which tasks or operations are executed, which can be synchronous or asynchronous. Synchronous model is the main choice for most distributed frameworks \cite{DBLP:conf/sigmod/MalewiczABDHLC10,DBLP:conf/ssdbm/SalihogluW13,}, since it is easy for programming and suits to most algorithms, particularly those based on iterative computations. While some frameworks \cite{DBLP:journals/pvldb/LowGKBGH12,DBLP:conf/cidr/WangXDG13,DBLP:conf/eurosys/ChenLZYYC18,DBLP:conf/icde/WangGHYH19,} choose asynchronous or hybrid model that allows a more flexible execution where vertices do not wait for each other and operate independently based on their received information.
This approach has greater efficiency, while increases the complexity of algorithms for ensuring the correctness. 

\underline{\textit{Communication.}} Communication in a distributed system refers to the method of message exchange between different units or vertices, main includes message passing and shared memory. Message passing is the main communication approach in distributed graph processing. Its main advantage is the flexibility it offers, which can enhance the scalability of the algorithm. However, for algorithms that require frequent exchanges of information with neighbors or need global information, this may pose the challenge communication overhead. 
The shared memory method allows data to be presented as shared variables, accessible for reading and modification by any vertices or program. This method abstracts the physical location and access mechanisms of data in memory, i.e., it simplifies data access by making it seem like data is locally available, regardless of its actual physical location. However, this approach also introduces challenges in maintaining data consistency. To ensure that all units have an accurate and updated data, effective synchronization and consistency mechanisms are necessary.
% These mechanisms must resolve conflicts from simultaneous read and write operations and balance the need for consistency with system performance.
% The shared memory method lets data expose as shared variables that can be directly read or be modified by any vertices or programs. It simplifies data access, while presents challenges of ensuring consistency in distributed environments.

\underline{\textit{Execution Model.}} The execution model defines the strategy for task execution across multiple vertices, which is a pivotal factor in achieving efficient processing. Beyond the Vertex-Centric model in TLAV frameworks, the Edge-Centric and Subgraph-Centric models offer enhancements in different aspects. The Edge-Centric model, pioneered by X-Stream \cite{DBLP:conf/sosp/RoyMZ13}, focuses on edges rather than vertices. This approach provides better performance for non-uniform graphs, especially those with power-law distributions, by streamlining interactions among edges and bypassing the random memory accesses associated with vertices \cite{DBLP:journals/csur/HeidariSCB18}. While the Edge-Centric model tends to be more complex to program, it offers enhanced performance for algorithms that require pre-processing of sorting edge lists, like BFS \cite{DBLP:journals/fgcs/ZhuHLM20, DBLP:conf/sosp/RoyMZ13}. The Subgraph-Centric model, encapsulated by the "think like a graph" abstraction, concentrates on entire subgraphs. This model minimizes communication overhead, making it ideal for tasks where frequent vertex interaction is crucial, such as in social network analysis. However, it is less effective for power-law graphs and relies heavily on advanced graph partitioning techniques \cite{DBLP:journals/tpds/ZhangJHLYY23, DBLP:journals/csur/BouhenniYNK21, DBLP:conf/sigmod/QuamarD16, DBLP:conf/ppopp/XieCGZC15}. Frameworks like Giraph++, GoFFish, and Blogel adapt this model \cite{DBLP:journals/pvldb/TianBCTM13, DBLP:conf/europar/SimmhanKWNRRP14, DBLP:journals/pvldb/YanCLN14}.



==> section/sec3_Graph_Algotithms.tex <==
Graphs possess a powerful ability to express relationships between entities. Many real-world applications can be represented as graph data, encompassing social networks, route planning, collaborative networks, and various others. 
As the scale of real-world graph data continues to grow and the processing capabilities of single machines become limited, numerous algorithms specifically designed for distributed systems have emerged. In this paper, we categorize these algorithms into seven distinct categories: Centrality, Graph Clustering/Community Detection, Similarity, Cohesive Subgraph/Community Search, Traversal, Pattern Matching, and Other. In this section, we will provide an introduction to these algorithms and further discuss and summarize the existing efforts in sections 4-10.

\subsection{Centrality}

Centrality is a widely used approach for quantifying the relative importance of each individual node in a complex graph. Nodes with high centrality value are more likely to have more edges, link to more nodes, and be closer to other nodes. Recently, distributed computation methods for centrality has arose attentions since the distributed framework is adept at the heavy computation, which is the major challenge in centrality computing.

\subsubsection{PageRank}
PageRank is one of the most popular algorithms to rank the importance of webpages, which can be modeled as a graph where each webpage is a node and each hyperlink is an edge.

The PageRank values, denoted by $\pi$, are the stationary probabilities of the following $\alpha$-decay random walk: it initially starts from a node chosen uniformly at random; at each step, with probability $\alpha$ it restarts at a random node, and with remaining probability $1-\alpha$ it walks to a random neighboring node. For each node $v$, the PageRank value of $u$ is denoted by $\pi(v)$. So the stationary state is:
\begin{equation}
    \pi(v) = (1 - \alpha) \cdot \frac{1}{n} + \alpha \cdot \sum_{u \in N_{in}(v)} \frac{\pi(u)}{N_{out}(u)}
\end{equation}

It is not ordinary to find such $\pi$ since it involves matrix inversion solving. Instead, recent researches often use an iterative form:
\begin{equation}
    \pi_{i+1}(v) = (1 - \alpha) \cdot \frac{1}{n} + \alpha \cdot \sum_{u \in N_{in}(v)} \frac{\pi_i(u)}{N_{out}(u)}
\end{equation}
In each iteration, all PageRank values are updated by the previous results, until convergence. 


\subsubsection{Personalized PageRank (PPR)}

Personalized PageRank (PPR) is similar to PageRank but PPR allows users to specify a start node $s$. When the random walk initially starts and with the probability $\alpha$ restarts, it will not choose a random node. Instead, it will always start at $s$. The equation can be modified to:
\begin{equation}
    \pi_{i+1}(v) = (1 - \alpha) \cdot e_s(v) + \alpha \cdot \sum_{u \in N_{in}(v)} \frac{\pi_i(u)}{N_{out}(u)}
\end{equation}
where $e_s$ is a one-hot vector and $e_s(v)=1$ if and only if $v=s$.

\subsubsection{Degree Centrality}

Degree Centrality is the historically first and conceptually simplest centrality indices, which is defined as the number of neighboring nodes:
\begin{equation}
    C_D(v) = \vert N(v) \vert = \deg (v)
\end{equation}
To eliminate the impact of the graph scale, a normalized form is more acceptable: 
\begin{equation}
    C_D(v) = \frac{\deg (v)}{n - 1}
\end{equation}

The computation of the degree centrality can be easily distributed since the degree value is a basic attribution.


\subsubsection{Betweenness Centrality}

The betweenness centrality counts the number of shortest paths a node located in. The main idea is that a more important node tend to dominate more shortest paths and control more communications. It has to divide a total number of node pairs to normalize:
\begin{equation}
    C_b(v) = \frac{1}{(n-1)(n-2)} \sum_{s,t \in V, s \neq v \neq t} \frac{\sigma_{st}(v)}{\sigma_{st}}
\end{equation}
where $\sigma_{st}$ is the number of shortest paths from $s$ to $t$, and $\sigma_{st}(v)$ is the number of such paths that includes $v$. The direct computation process of the betweenness centrality involves All pairs Shortest paths (APSP) counting, which costs $\vert V \vert ^2 \log \vert V \vert + \vert V \vert \vert E \vert$ on a weighted graph or $\vert V \vert \vert E \vert$ on a unweighted graph.

\subsubsection{Closeness Centrality}

The closeness centrality measures the average length of the shortest path from the node to all other nodes, which means a more important node will be closer to others. A normalized form of the closeness centrality is:
\begin{equation}
    C_c(v) = \frac{n-1}{\sum_{u \in V} d(v, u)}
\end{equation}

\subsection{Graph Clustering/Community Detection}

Community detection (or graph clustering) is a fundamental problem in the field of graph data mining, which goal is to partition the vertices in the graph into different clusters (communities), where the vertices within a cluster (community) are more densely connected to each other than to those outside the cluster (community). 


\subsubsection{Louvain}
Louvain \cite{blondel2008fast} is a modularity-based community detection algorithm and is widely regarded as one of the most popular methods in this field. Modularity $Q$ is usually employed to assess the quality of communities, which is defined as,

\begin{equation}
    Q = \frac{1}{2m}\sum_{i,j}\left[A_{ij} - \frac{k_ik_j}{2m}\right]\delta(c_i,c_j)
\end{equation}

where $A_{ij}$ represents the weight of the edge$(i, j)$, $k_i  = \sum_{j}A_{ij}$ is the sum of weights of the edges attached to vertex $i$, $c_i$ is the community including vertex $i$, the function $\delta$ is 1 if $u = v$ and 0 otherwise, and $m = \frac{1}{2}\sum_{ij}A_{ij}$.

\subsubsection{Label Propagation} 
The Label Propagation algorithm (LPA) \cite{raghavan2007near} is an effective approach to detect communities by propagating labels throughout the network. The algorithm starts by assigning a unique community label to each vertex, and then these labels propagate through the network. At each iteration, a vertex updates its label to the one that the maximum number of its neighbors belongs to, until it reaches convergence where every vertex has the majority label of its neighbors. LPA will stop either when convergence is achieved or when the maximum number of iterations defined by the user is reached. 

The attraction of LPA is that it does not require any prior information and has a linear running time. Its time complexity in a single machine is $O(k\cdot m)$, where $m$ is the number of edges in the graph and $k$ is the maximum number of iterations.


\subsubsection{Minimum Cut/Max Flow} 
The minimum cut algorithm and max flow algorithm are well-known algorithms in graph theory. The former aims to divide the vertices of the graph into two mutually exclusive subsets while minimizing the sum of edge weights between the two subsets, and the later aims to find as much as feasible flow from the source node $s$ to the sink node $t$ in a graph, in which each edge has a flow capacity. Although they are defined differently, the problems they address can be considered as belonging to the same category, i.e., they are dual problems to each other.
The algorithm has broad applications in various fields, including community detection, natural language processing, and data segmentation in distributed systems. However, solving this problem can be computationally intensive and the time complexity for solving this problem on a single machine is $O(n^2logn)$, where $n$ is the number of vertices in the graph \cite{DBLP:conf/soda/Karger93}.


\subsubsection{Connected Components}
Computing connected components is one of the most fundamental and widely studied problems in the field of graph analytics.
The connected components of an undirected graph can be defined as subgraphs in which every vertex is reachable from every other vertex within the same subgraph. In contrast, strongly connected components in a directed graph are subgraphs where there is a directed path between any two vertices, while in the case of a weakly connected component, it can be seen as connected components in the undirected graph that is obtained by replacing all directed edges with undirected edges.


\subsubsection{Local Clustering Coefficient} The Local Clustering Coefficient is a measure used to gauge the density of connections between a node and its adjacent nodes. It indicates the ratio of the number of real connections among the node's neighbors to the possible number of connections.


\subsection{Similarity}

The similarity algorithm measures the similarity between two vertices, which usually exams their shared neighbors. This algorithm is widely used in various fields such as social network analysis, recommendation systems, and anomaly detection. 
% Common similarity algorithms include Cosine Similarity, Jaccard Similarity, and SimRank.
Moreover, the calculation of the similarity algorithm has locality. This means that it only needs to consider the local part of the graph rather than the entire that. This feature makes it suitable for distributed computing, especially when dealing with large-scale graphs.

\subsubsection{Jaccard Similarity} 
Jaccard similarity measures the similarity between two sets based on their shared elements. Specifically, it is defined as the size of the intersection of two sets divided by the size of their union, which is:

\begin{equation}
    Jaccard(A, B) = \frac{|A \cap B|}{|A \cup B|}
\end{equation}

The value of Jaccard similarity ranges from 0 to 1, and if either $A$ or $B$ is an empty set, the value is 0. In graph data, set A or B is usually considered as the set of all neighbors of a certain vertex.


\subsubsection{Cosine Similarity} Cosine similarity originally is a measure of similarity between two non-zero vectors, which is defined as,

\begin{equation}
    Cosine(a, b) = \frac{a \cdot b}{|a| \times |b|}
\end{equation}

where $a$ and $b$ are n-dimensional vectors.

In the field of graph data, there is also a similar measure, which is also called Otsuka–Ochiai Coefficient, which is defined as,

\begin{equation}
    Cosine(A, B) = \frac{|A \cap B|}{\sqrt{|A| \times |B|}}
\end{equation}

Similar to Jaccard similarity, A or B is usually considered as the set of all neighbors of a certain vertex.

\subsubsection{SimRank} The SimRank algorithm is based on the observation that "two objects are considered similar if they are referenced by similar objects" \cite{DBLP:conf/kdd/JehW02}, i.e., the similarity of a vertex is determined by the similarity of its neighbors. The formal definition of SimRank is,

\begin{equation}
    s(a, b) = \frac{C}{|I(a)|\cdot|I(b)|}\sum_{i=1}^{|I(a)|}\sum_{j=1}^{|I(b)|}s(I_i(a), I_j(b))
\end{equation}

where $C$ is a constant between 0 and 1, and the set of in-neighbors of $a/b$ is denoted as $I(a)/I(b)$, where $I_i(a)/I_j(b)$ represent the $i$-th$/$$j$-th in-neighbor of $a/b$. Note that $s(a,b)=1$ if $a=b$ and $s(a,b)=1$ when $I(a)=\emptyset$ or $I(b)=\emptyset$.


% \subsection{123}
\subsection{Cohesive Subgraph/Community Search}

Community networks are a prevalent and significant structure in large-scale graphs, such as social networks, biological networks, financial transaction networks. Essentially, a community refers to a group made up of interconnected vertices that often share common characteristics or attributes. Retrieving communities from a graph (community search) is one of the fundamental problems in graph computing science \cite{DBLP:conf/icde/HuangLX17}, which aims to search communities regarding query vertices or some query parameters \cite{DBLP:journals/vldb/FangHQZZCL20}. 
The primary community search algorithms include ($k$-core decomposition, $k$-truss, $k$-clique and $k$-ECC).

Another research work, called community detection, is highly related to community search, but their problem definitions, criteria of defining communities and algorithms are different according to \cite{DBLP:journals/vldb/FangHQZZCL20}. Compared to community detection, the communities found through community search are more dependent on query parameters given by the users rather than the graph's inherent properties.


% {\color{red}(If there are other comparisons, summaries, or classifications included later in this section, these expressions need to be modified.)}

\subsubsection{$K$-Core Decomposition} 
The $k$-core is one of the most significant and widely researched cohesive subgraphs, defined as the maximal subgraph of the original graph where each vertex in this subgraph has a degree of at least $k$ \cite{DBLP:journals/vldb/MalliarosGPV20}. $k$-core decomposition is the process of computing $k$-core communities, which recursively delete all vertices (and edges connected to them) with a degree less than $k$ until the degree of each remaining vertex is no less than $k$. In a single-machine scenario, the process takes $O(m + n)$ time and $O(m + n)$ space. The $k$-core has been extensively used in various network analyses, including social networks and protein-protein interaction networks, due to its easily computable nature with linear time complexity.


\subsubsection{$K$-Truss} A $k$-truss is the maximal subgraph of the original graph in which each edge is contained in at least $(k-2)$ triangles. The cohesiveness of $k$-truss community is higher than $k$-core and $k$-ECC but less than $k$-clique since it is defined on the basis of triangles \cite{DBLP:journals/vldb/FangHQZZCL20,DBLP:conf/bigdataconf/ChenCC14}. Similar to $k$-core, the k-truss decomposition algorithm can be employed to compute the k-truss community, which recursively delete all edges which trussness is less than $k$ until each remaining edge is contained in at least $(k-2)$ triangles. In a single-machine scenario, the time complexity of computing a $k$-truss community is bounded by $O(m^{1.5})$, which is primarily spent on computing all triangles. 


\subsubsection{$K$-Clique} 
A $k$-clique is a set of $k$ vertices in the original graph where each pair of vertices has an edge. The $k$-clique community has the highest level of cohesiveness among all cohesive subgraphs, and its time complexity on a single machine is also the highest. 
The clique-related problems also include other two types: maximal clique and maximum clique. The former represents all cliques which cannot be extended by any other vertex, while the later represents the largest clique, i.e., the maximal clique which has the largest size.
Enumerating all maximal cliques and maximum cliques require $O(3^{n/3})$ and $O(2^{0.249n})$ time, respectively, in the worst case \cite{DBLP:journals/tkde/ShahrivariJ21}. The conclusion of $k$-clique is easier, but it still requires $O(k^2n^k)$ time. Clearly, all of these problems are NP-hard.
% {\color{red}(if biclique is added in here)}

\subsubsection{$K$-ECC} A $k$-ECC (k-edge-connected component) is a subgraph of the original graph in which after removing any $k-1$ edges, it is still connected. 
% According to \cite{DBLP:conf/sigmod/ChangLQYZ15}, it takes $O(|V|\cdot h\cdot l\cdot|E|)$ time if the $k$-ECC enumeration algorithm is based on graph decomposition or $O(|V|\cdot t\cdot|E|)$ time if that is based on the random contraction.
Existing methods for computing on a single machine need at least $O(h\cdot l\cdot |E|)$ time, where $l$ is a small integer with $l \ll|V|$ and $h$ reflects the "depth" of the $k$-ECC nested together to form the graph \cite{DBLP:conf/sigmod/ChangYQLLL13}.


\subsection{Traversal}

The traversal algorithm typically adheres to specific rules or orders to access each vertex or edge in a graph sequentially, allowing it to execute a particular operation or retrieve crucial information.

\subsubsection{Breadth-First-Search (BFS) and Depth-First-Search (BFS)}

BFS starts at a source node, exploring all vertices at the current depth and then visiting the next layer. This hierarchical structure can help to find the shortest path, i.e., Single Source Shortest Path (SSSP). Moreover, BFS can help to find the feasible flow in the maximum flow problem. Another example is the Minimum Spanning Tree (MST), which is often solved by Borůvka's algorithm in distributed environment and needs graph traversal to find the shortest edge.

DFS also starts at the given source node, exploring as far as possible before backtracking. This no-repeat and single-direction property can help to detect cycles in a graph, i.e., cycle detection problem.

The challenge of BFS/DFS is that the process may visit some vertices more than once, since it is not known whether a vertex is visited before the transition. Therefore, the efficiency highly depend on the graph density and the redundancy is prevalent in a dense graph.
The total time complexity of BFS/DFS is fixed as $O(n+m)$ but the real execute time is highly affected by the implementation and optimizations. 

\subsubsection{Single Source Shortest Path}

The Single Source Shortest Path (SSSP) problem requires to find the shortest path from a source node to other vertices. In unweighted graph, the shortest path distance equals to the number of layers. So SSSP focus on the weighted graph.

Dijkstra's algorithm is the most widely used SSSP algorithm with single thread. However, Dijkstra's algorithm involves a heap to maintain the current distances, which is hard to parallelize and migrate to a distributed platform. The lower bound had been proved as $\widetilde{Omega}(D + \sqrt{n})$, but no specific implementation can reach the theoretical bound.

\subsubsection{Minimum Spanning Tree}

Minimum Spanning Tree (MST) refers to finding a tree that contains all vertices in a connected graph, and the sum of the weights of all edges in the tree is minimized.
This algorithm measures the connecting cost of a graph. Traditional method including Prim's algorithm and Kruskal's algorithm rely on a priority queue and not intuitive to be distributed. 


\subsubsection{Cycle Detection}

The cycle detection algorithm refers to the process of checking whether a specific cycle structure, a path that starts from a vertex and eventually returns to the same vertex, exists in a graph.


\subsection{Pattern Matching}


\subsubsection{Triangle Counting}
A triangle is a clique formed by 3 vertices. Triangles are the fundamental structure in a graph and the problem of counting triangles has been widely studied. Triangle counting has important applications in various fields such as social and biological network analysis, network flow optimization, recommendation systems and more. The famous cohesive subgraph $k$-truss is the maximum subgraph where every edge appears in at least $k-2$ triangles and the similarity between two adjacent vertices in structural clustering is also measured by the number of common neighbors (i.e. the number of triangles). Additionally, triangle counting is also a crucial step in calculating the local clustering coefficient, a popular measure of clustering in graphs.


\subsubsection{Subgraph Matching}


\subsection{Other}

\subsubsection{Maximum Independent Set} 

An independent set is a set of vertices in a graph where no two vertices are directly connected. The maximum independent set is an independent set that is not a subset of any other independent set. The maximal independent set can be seen as the maximum independent set with the largest number of vertices. However, computing the maximum/maximal independent set is a challenging task that falls under the NP-hard problem category. To efficiently solve this problem in practical applications, heuristic algorithms or approximation algorithms are often used. To handle large-scale graphs, deploying the algorithm to distributed clusters is an effective approach. However, communication and load balancing pose significant challenges in a distributed environment because of the extensive amount of communication required between vertices. Moreover, the computation of the maximum independent set on a single machine requires consideration of the entire graph structure, which further complicates the distributed implementation.


\subsubsection{Coloring}
The coloring problem is assigning distinct colors to all vertices (or edges) in a graph, ensuring that neighboring vertices (or edges) do not have the same color. This problem has significant applications in various fields, including map coloring, scheduling problems, and compiler optimization.
Assigning colors to a graph using the minimum number of colors is an NP-hard problem.
Distributed solutions to the coloring problem are a very meaningful research direction. According to the research of Gandhi et al. \cite{DBLP:conf/iccnc/GandhiM15}, the algorithms base on distributed models like BSP  perform better than heuristic based algorithms. However, the challenge of more communication and computation overhead still remains.


==> tikzlibrarypie.code.tex <==
% SPDX-License-Identifier: GPL-2.0-only OR LPPL-1.3c
\RequirePackage{scalefnt}

%
% Utilities
%

\def\pgfpie@ifx#1#2{%
  \ifx#1#2%
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifdim#1#2#3{%
  \ifdim\dimexpr#1\relax#2\dimexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifnum#1#2#3{%
  \ifnum\numexpr#1\relax#2\numexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifodd#1{%
  \ifodd\numexpr#1\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@newif#1{%
  \csname newif\expandafter\endcsname\csname ifpgfpie@#1\endcsname
  \expandafter\def\csname pgfpie@if#1\expandafter\endcsname\expandafter{%
    \csname ifpgfpie@#1\endcsname
      \expandafter\pgfutil@firstoftwo
    \else
      \expandafter\pgfutil@secondoftwo
    \fi}%
}

%
% Constants for text comparison
%

\def\pgfpie@text@inside{inside}
\def\pgfpie@text@legend{legend}
\def\pgfpie@sum@c{100}
\def\pgfpie@sum@auto{auto}

% args:
% #1: begin angle
% #2: end angle
% #3: number
% #4: label
% #5: explode
% #6: fill color
% #7: radius
% #8: center
\def\pgfpie@slice#1#2#3#4#5#6#7#8{%
  \pgfmathparse{0.5*(#1)+0.5*(#2)}
  \let\pgfpie@midangle\pgfmathresult

  \path (#8) -- ++({\pgfpie@midangle}:{#5}) coordinate (pgfpie@O);

  \pgfmathparse{(#7)+(#5)}
  \let\pgfpie@radius\pgfmathresult
  
  % slice
  \draw[line join=round,fill={#6},\pgfpie@style] (pgfpie@O) -- ++({#1}:{#7}) arc ({#1}:{#2}:{#7}) -- cycle;

  \pgfpie@ifchangedirection{%
    \pgfmathparse{min(((#1)-(#2)-10)/110*(-0.3),0)}
  }{%
    \pgfmathparse{min(((#2)-(#1)-10)/110*(-0.3),0)}
  }%
  
  \pgfmathparse{(max(\pgfmathresult,-0.5) + 0.8)*(#7)}
  \let\pgfpie@innerpos\pgfmathresult

  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    % label and number together
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#4}\\\pgfpie@numbertext{#3}};
  }{%
    % label
    \pgfpie@ifhidelabel{}{%
      \pgfpie@iflegend{}{%
        \path (pgfpie@O) -- ++ ({\pgfpie@midangle}:{\pgfpie@radius})
        node[inner sep=0, \pgfpie@text={\pgfpie@midangle:#4}]{};
      }%
    }%

    % number
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\def\pgfpie@findColor#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@colorLength))}%
  \let\pgfpie@ci\pgfmathresult
  \foreach \pgfpie@c [count=\pgfpie@j from 0] in \pgfpie@color {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ci}{%
      \xdef\pgfpie@thecolor{\pgfpie@c}%
      \breakforeach
    }{}%
  }
}

\def\pgfpie@findExplode#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@explodeLength))}%
  \let\pgfpie@ei\pgfmathresult
  \foreach \pgfpie@e [count=\pgfpie@j from 0] in \pgfpie@explode {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ei}{%
      \xdef\pgfpie@theexplode{\pgfpie@e}%
      \breakforeach
    }{}%
  }%
}

% #1: bottom left point
% #2: size
% #3: number
% #4: color
% #5: text
\def\pgfpie@square#1#2#3#4#5{%
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#5}\\\pgfpie@numbertext{#3}} ++(#2);
  }{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}} ++(#2);
  }%
}

% #1: pos
% #2: radius
% #3: number
% #4: color
% $5: style
% $6: label
\def\pgfpie@cloud#1#2#3#4#5#6{%
  \draw[fill=#4, #5] (#1) circle[radius=#2];
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \node[align=center] at (#1) {\pgfpie@scalefont{#3}\pgfpie@labeltext{#6}\\\pgfpie@numbertext{#3}};
  }{%
    \node at (#1) {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\newdimen\pgfpie@angleEnd
\newcount\pgfpie@explodeLength
\newcount\pgfpie@colorLength
\newcount\pgfpie@sliceLength

\pgfqkeys{/pgfpie}{%
  .search also={/tikz,/pgf},
  explode/.store in=\pgfpie@explode,
  color/.store in=\pgfpie@color,
  radius/.store in=\pgfpie@radius,
  pos/.store in=\pgfpie@pos,
  style/.store in=\pgfpie@style,
  before number/.store in=\pgfpie@beforenumber,
  after number/.code={%
    \def\pgfpie@afternumber{#1}%
    \def\pgfpie@late@afternumber{}%
  },
  text/.store in=\pgfpie@text,
  sum/.code={%
    \def\pgfpie@sum{#1}%
    \pgfpie@ifx\pgfpie@sum\pgfpie@sum@c{%
      \def\pgfpie@late@afternumber{\def\pgfpie@afternumber{\%}}%
    }{%
      \def\pgfpie@late@afternumber{}%
    }%
  },
  rotate/.store in=\pgfpie@rotate,
}

\pgfpie@newif{polar}
\pgfqkeys{/pgfpie}{polar/.is if=pgfpie@polar}

\pgfpie@newif{legend}

\pgfpie@newif{changedirection}
\pgfqkeys{/pgfpie}{change direction/.is if=pgfpie@changedirection}

\pgfpie@newif{square}
\pgfqkeys{/pgfpie}{square/.is if=pgfpie@square}

\pgfpie@newif{cloud}
\pgfqkeys{/pgfpie}{cloud/.is if=pgfpie@cloud}

\pgfpie@newif{scalefont}
\pgfqkeys{/pgfpie}{scale font/.is if=pgfpie@scalefont}
\def\pgfpie@scalefont#1{%
  \pgfpie@ifscalefont{%
    \pgfmathparse{(#1) / (\pgfpie@sum) * 3 + 0.9}%
    \scalefont{\pgfmathresult}%
  }{}%
}

\pgfpie@newif{hidenumber}
\pgfqkeys{/pgfpie}{hide number/.is if=pgfpie@hidenumber}
\def\pgfpie@numbertext#1{%
  \pgfpie@ifhidenumber{}{%
    \pgfpie@beforenumber#1\pgfpie@afternumber
  }%
}

\pgfpie@newif{hidelabel}
\pgfqkeys{/pgfpie}{hide label/.is if=pgfpie@hidelabel}
\def\pgfpie@labeltext#1{\pgfpie@ifhidelabel{}{#1}}

\tikzaddtikzonlycommandshortcutlet{\pie}{\pgfpie@pie}%

\def\pgfpie@pie{%
  \pgfutil@ifnextchar[{\pgfpie@@pie}{\pgfpie@@pie[]}%
}

\def\pgfpie@@pie[#1]#2{%
  \scope[%
    % to be compatible with "babel" lib
    handle active characters in nodes=false,
    % load default parameters
    /pgfpie/.cd,
    explode=0,
    color={blue!60, cyan!60, yellow!60, orange!60, red!60,
      blue!60!cyan!60, cyan!60!yellow!60, red!60!cyan!60,
      red!60!blue!60, orange!60!cyan!60},
    radius=3,
    pos={0,0},
    style={thick},
    before number=,
    after number=,
    text=label,
    sum=100,
    rotate=0,
    change direction=false,
    polar=false,
    square=false,
    cloud=false,
    scale font=false,
    hide number=false,
    hide label=false,
    every pie/.try,%
    % load user's parameters
    #1]

  % add percentage automatically
  \pgfpie@late@afternumber

  % legend or not
  \pgfpie@ifx\pgfpie@text\pgfpie@text@legend{%
    \pgfpie@legendtrue
  }{%
    \pgfpie@legendfalse
  }%

  % handle sum
  \pgfpie@ifx\pgfpie@sum\pgfpie@sum@auto{%
    % sum all input
    \xdef\pgfpie@sum{0}%
    \foreach \pgfpie@p/\pgfpie@t in {#2} {%
      \pgfmathparse{(\pgfpie@sum) + (\pgfpie@p)}%
      \xdef\pgfpie@sum{\pgfmathresult}%
    }%
  }{}%

  % init counters
  \global\pgfpie@explodeLength=0
  \foreach \pgfpie@e in \pgfpie@explode {%
    \global\advance\pgfpie@explodeLength by 1
  }%

  \global\pgfpie@colorLength=0
  \foreach \pgfpie@c in \pgfpie@color {%
    \global\advance\pgfpie@colorLength by 1
  }%
  
  \pgfmathsetlength{\pgfpie@angleEnd}{0}%

  \global\pgfpie@sliceLength=0
  \foreach \pgfpie@p/\pgfpie@e in {#2} {%
    \global\advance\pgfpie@sliceLength by 1
  }%

  \pgfpie@ifsquare{%
    \pgfpie@pie@square{#2}%
    }{\pgfpie@ifcloud{\pgfpie@pie@cloud{#2}%
      }{\pgfpie@pie@circle{#2}}}

  % legend
  \pgfpie@ifhidelabel{}{%
    \pgfpie@iflegend{%
      \pgfpie@legend{#2}%
  }{}}%
  \endscope
}

\def\pgfpie@pie@square#1{%
  \pgfmathparse{(\pgfpie@radius)*2}
  \xdef\pgfpie@verticalLength{\pgfmathresult}
  \xdef\pgfpie@horizontalLength{\pgfmathresult}
  \path (\pgfpie@pos) -- ++({-\pgfpie@radius},{-\pgfpie@radius}) coordinate (pgfpie@start);
  \pgfmathparse{(\pgfpie@verticalLength) * (\pgfpie@horizontalLength) / (\pgfpie@sum)}
  \let\pgfpie@squareUnit\pgfmathresult

  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@ifdim{\pgfpie@verticalLength cm}{>}{\pgfpie@horizontalLength cm}{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@horizontalLength)}
      \let\pgfpie@height\pgfmathresult
      
      \pgfpie@square{pgfpie@start}{\pgfpie@horizontalLength,\pgfpie@height}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@horizontalLength},{\pgfpie@height*0.5})
            node[inner sep=0, \pgfpie@text={0:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{\pgfpie@verticalLength - \pgfpie@height}
      \xdef\pgfpie@verticalLength{\pgfmathresult}
      \path (pgfpie@start) -- ++(0, \pgfpie@height) coordinate (pgfpie@start);
    }{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@verticalLength)}%
      \let\pgfpie@width\pgfmathresult

      \pgfpie@square{pgfpie@start}{\pgfpie@width,\pgfpie@verticalLength}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@width*0.5},{\pgfpie@verticalLength})
            node[inner sep=0, \pgfpie@text={90:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{(\pgfpie@horizontalLength) - (\pgfpie@width)}%
      \xdef\pgfpie@horizontalLength{\pgfmathresult}%
      \path (pgfpie@start) -- ++({\pgfpie@width},0) coordinate (pgfpie@start);
    }%
  }%
}

\def\pgfpie@pie@cloud#1{%
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    % find explode
    \pgfpie@findExplode{\pgfpie@i}
    \def\pgfpie@cloudGap{(\pgfpie@theexplode) + 0.1}
    \pgfmathparse{sqrt((\pgfpie@p) / (\pgfpie@sum)) * (\pgfpie@radius)}
    \let\pgfpie@cloudR\pgfmathresult
    \pgfpie@ifnum{\pgfpie@i}{=}{0}{%
      % first cloud
      \coordinate (pgfpie@O) at (\pgfpie@pos);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{180+(\pgfpie@rotate)}
    }{\pgfpie@ifnum{\pgfpie@i}{=}{1}{%
      % second cloud
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{45+(\pgfpie@rotate)}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}) coordinate (pgfpie@O);
    }{%
      % next cloud
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}
      \let\pgfpie@la\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lb\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRtwo)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lc\pgfmathresult
      \pgfmathparse{(\pgfpie@la)^2+(\pgfpie@lc)^2-(\pgfpie@lb)^2}
      \let\pgfpie@tmp\pgfmathresult
      \pgfmathparse{180 - acos((\pgfpie@tmp) / 2 / (\pgfpie@la) / (\pgfpie@lc))}
      \let\pgfpie@cloudRot\pgfmathresult
      \pgfpie@ifodd{\pgfpie@i}{%
        \pgfmathparse{-(\pgfpie@cloudRot)}
        \let\pgfpie@cloudRot\pgfmathresult
      }{}%
      \pgfmathparse{(\pgfpie@cloudExtendDir) - (\pgfpie@cloudRot)}
      \xdef\pgfpie@cloudExtendDir{\pgfmathresult}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@lc}) coordinate (pgfpie@O);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudRtwo}
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
    }}%

    % find color
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@cloud{pgfpie@O}{\pgfpie@cloudR}{\pgfpie@p}
    {\pgfpie@thecolor}{\pgfpie@style}{\pgfpie@t}

    % label
    \pgfpie@iflegend{}{%
      \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
        \pgfpie@ifhidelabel{}{%
          \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@cloudR})
          node[inner sep=0, \pgfpie@text={\pgfpie@cloudExtendDir:{\pgfpie@t}}] {};
        }%
      }%
    }%
  }%
}

\def\pgfpie@pie@circle#1{%
  \pgfpie@ifpolar{%
    \xdef\pgfpie@maxValue{0}
    \foreach \pgfpie@p/\pgfpie@e in {#1} {
      \pgfmathparse{\pgfpie@p}%
      \pgfpie@ifdim{\pgfpie@maxValue pt}{<}{\pgfmathresult pt}{%
        \xdef\pgfpie@maxValue{\pgfpie@p}
      }{}%
    }
    \pgfmathparse{(\pgfpie@sum) / \the\pgfpie@sliceLength}
    \xdef\pgfpie@polarangle{\pgfmathresult}
    \pgfmathparse{(\pgfpie@radius) / sqrt(\pgfpie@maxValue)}
    \xdef\pgfpie@polarRadiusUnit{\pgfmathresult}
  }{%
    \xdef\pgfpie@theradius{\pgfpie@radius}%
  }

  \pgfpie@ifchangedirection{%
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@sum}
  }{}%
  \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@angleBegin}
    \pgfpie@ifpolar{%
      % Polar area diagram
      \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@polarangle}
      \pgfmathparse{sqrt(\pgfpie@p) * (\pgfpie@polarRadiusUnit)}
      \xdef\pgfpie@theradius{\pgfmathresult}
    }{%
      % normal pie
      \pgfpie@ifchangedirection{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{-(\pgfpie@p)}
      }{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@p}
      }%
    }%

    % find explode
    \pgfpie@findExplode{\pgfpie@i}

    % find color
    \pgfpie@findColor{\pgfpie@i}
    \pgfpie@slice{(\pgfpie@angleBegin)/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\the\pgfpie@angleEnd/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\pgfpie@p}
    {\pgfpie@t}
    {\pgfpie@theexplode}
    {\pgfpie@thecolor}
    {\pgfpie@theradius}
    {\pgfpie@pos}
    \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  }
}

\def\pgfpie@legend#1{%
  \coordinate[xshift=0.8cm,
  yshift={(\the\pgfpie@sliceLength*0.5+1)*0.5cm}] (pgfpie@legendpos) at
  (current bounding box.east);

  \scope[node distance=0.5cm]
    \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
    {
      \pgfpie@findColor{\pgfpie@i}
      \node[draw, fill={\pgfpie@thecolor}, \pgfpie@style, below of={pgfpie@legendpos}, label={0:{\pgfpie@t}}] (pgfpie@legendpos) {};
    }
  \endscope
}

